Specializing Coherence, Consistency, and Push/Pull for GPU Graph Analytics

This work provides the first study to explore the interaction of update propagation with and without fine-grained synchronization (push vs. pull), emerging coherence protocols (GPU vs. DeNovo coherence), and software-centric consistency models (DRF0, DRF1, and DRFrlx) for graph workloads on emerging integrated GPU-CPU systems with native unified shared memory. We study 6 graph applications with 6 graph inputs for a total of 36 workloads running on 12 system (hardware+software) configurations reflecting the above design space of update propagation, coherence, and memory consistency. We make three key contributions. First, we show that there is no single best system configuration for all workloads, motivating systems with flexible coherence and consistency support. Second, we develop a model to accurately predict the best system configuration -- this model can be used by software designers to decide on push vs. pull and the consistency model and by flexible hardware to invoke the appropriate coherence and consistency configuration for the given workload. Third, we show that the design dimensions explored here are inter-dependent, reinforcing the need for software-hardware co-design in the above design dimensions. For example, software designers deciding on push vs. pull must consider the consistency model supported by hardware -- in some cases, push maybe better if hardware supports DRFrlx while pull may be better if hardware does not support DRFrlx.

==> applications.tex <==
\section{Applications}
\label{sec:applications}

  \subsection{PageRank~(PR)}
  \label{subsec:applications-pr}

  \subsection{Single-Source Shortest Path~(SSSP)}
  \label{subsec:applications-sssp}

  \subsection{Graph Coloring~(CLR)}
  \label{subsec:applications-clr}

  \subsection{Maximal Independent Set~(MIS)}
  \label{subsec:applications-mis}


==> background.tex <==
\section{Background}
\label{sec:background}

To motivate the use of GPUs for the acceleration of parallel graph analytics workloads, we first describe the benefits and challenges faced by application developers targeting GPUs for these workloads.
% Then, we demonstrate the relationship between implementation choice and locality, synchronization, and input-dependence.
% Finally, we explain the state-of-the-art for GPU coherence and consistency, as motivated by the demands of these emerging workloads.

  \subsection{Emerging GPU Applications}
  \label{subsec:background-gpu-emerging}

  As general purpose GPU programming matures, GPUs are being increasingly used for applications other than the traditional regular, streaming workloads~\cite{CheBoyer2009,StrattonRodrigues2012}.
  In contrast to regular GPU workloads, emerging, irregular applications suffer from both control and memory divergence.
%   While regular GPU workloads have well-understood control-flow, memory access, and synchronization patterns~\cite{CheBoyer2009,CheSheaffer2010}, emerging GPU workloads exhibit more irregular patterns.
%   The irregularity of emerging applications is important because of control divergence and memory divergence issues introduced when GPU architectures were unified using SIMT execution~\cite{LindholmNickolls2008,AMDGCNWhitePaper2012}
  Control divergence occurs when threads in the same \textit{warp}~(in CUDA) take different paths in the program due to input-dependence.
  Due to the SIMT scheduling granularity, resources in the GPU pipeline become underutilized when control divergence occurs.
  Memory divergence occurs when threads in the same warp make memory requests to disparate cache lines, or when requests from the same warp to the same cache lines cannot otherwise be coalesced.
  This form of divergence increases pressure on the memory system and may result in increased latency for memory accesses.

  Graph analytics applications on GPUs are an example of a workload that exhibits irregular control and memory access patterns~\cite{XuJeon2014}.  
%   Several benchmark suites for irregular GPU applications have been released, including Pannotia~\cite{CheBeckmann2013} and LonestarGPU~\cite{BurtscherNasre2012}, and graph analytics has been well studied on GPUs~\cite{BurtscherNasre2012,XuJeon2014}.
%   These kinds of graph analytics benchmarks have been studied in this context since irregularity introduces these overheads in GPUs~\cite{BurtscherNasre2012,XuJeon2014}.
%   However, graph analytics is still an attractive domain for GPU acceleration due to the parallelism present in many of these applications~\cite{CheBoyer2009}.
%   Moreover, these applications benefit from acceleration on tightly-coupled heterogeneous systems because of reduced communication and synchronization overheads~\cite{HestnessKeckler2015}.
  \textit{Topology-driven}, \textit{vertex-centric} implementations~\cite{CheBoyer2009,KimBatten2014,KhorasaniVora2014} of graph algorithms are commonly used because they are easy to implement and can achieve high throughput on GPUs via their asynchronous thread structure.
  A significant algorithmic design choice affecting these implementations is that of \textit{push} vs.\ \textit{pull}~\cite{BestaPodstawski2017}, as shown in Figure~\ref{alg:push-pull}.
  For kernels of graph algorithms that need to perform edge-propagated updates, a source vertex can either pull changes \emph{from} its neighbors or push changes \emph{to} its neighbors.
  For a given algorithm, both choices preserve the direction of the edge-propagated updates through the edge, but can change the control-flow and memory access behavior of the implementation.
  More importantly, pull does not require fine-grained synchronization while push does. Put another way, pull updates have no~\emph{races} while push updates do.
%   However, these implementations still suffer from control and memory divergence, which leads to workload imbalance. This imbalance motivates the need to quickly finish off long-latency tasks by exploiting instruction-level parallelism~(ILP) and memory-level parallelism~(MLP).
%   We only consider vertex-centric implementations throughout the rest of this paper.
  
%   A significant algorithmic design choice affecting both of these workload imbalance mitigating techniques is that of \textit{push} vs \textit{pull}.
%   For kernels of graph algorithms that need to perform edge-propagated updates, a source vertex can either pull changes \emph{from} its neighbors, or push changes \emph{to} its neighbors.
%   changes can either be propagated from a source vertex to a destination vertex (push), or grabbed from a destination vertex by a source vertex (pull).
%   For kernels of a graph algorithm which need to perform edge-propagated updates from the source vertex to the destination vertex of each edge in the graph, the application developer has the choice of whether the compute is mapped to the location of the source or destination vertex data.
%   Mapping the compute at the location of the source vertex data is a \textit{push-based} approach, while mapping the compute at the location of the destination vertex data is a \textit{pull-based} approach.
%   For a given algorithm, both choices preserve the direction of the edge-propagated updates through the edge, but can change the control-flow and memory access behavior of the implementation.
%   More importantly, pull does not require fine-grained synchronization while push does.
  
%   One of the critical properties of the push-pull dichotomy when parallelizing a vertex-centric implementation is that pull does not require fine-grained synchronization for kernels with edge-propagated updates, while push does.
%   When the computation is mapped to the location of the destination vertex data, a single thread can be responsible for the writes to a destination's new value, given that update information flows from the source vertex to the destination.
%   On the other hand, if the computation is mapped to the location of the source vertex data, several threads may attempt racy writes to the some shared destination vertices.
%   This means that a pull-implementation can forego fine-grained synchronization, while a push-implementation cannot.

  The push-pull dichotomy has been explored by prior work in the context of shared memory and distributed memory CPU systems~\cite{BestaPodstawski2017}.
  However, traditional GPU architectures suffer from unique challenges~(discussed further in Section~\ref{subsec:background-memory-systems}) which cause fine-grained synchronization to be performance prohibitive.
  Motivated by these challenges, recent work has explored multi-granular synchronization~\cite{LiBecchi2013,NasreBurtscher2013,KaleemVenkat2016} and synchronization-avoiding GPU techniques~\cite{NasreBurtscher2013}.
  Despite attempts to avoid synchronization, no work, to our knowledge, has reevaluated the push-pull dichotomy in light of new developments in GPU coherence and consistency.
  Moreover, sensitivity to input graph structure influences the trade-offs between locality, fine-grained synchronization, and workload imbalance.
  
%   We believe that a methodical assessment of the algorithmic and input-dependent properties of graph analytics workloads on GPUs is crucial for system designers who want to maximize performance when exploring the design space of these three dimensions: push-pull, GPU coherence, and GPU consistency.
  
%  \note{How much of this background section sounds like it needs to go in the introduction? Does the final motivation/setup for the taxonomy belong at the end of this section? Change the title of the section from ``Background'' to ``Motivation''?}

  %While previous works have characterized GPU graph analytics in the context of control-flow irregularity, memory access irregularity, synchronization costs, and input-sensitivity, no work to our knowledge has done so w.r.t 3 knobs ... \cite{TODO2,AhmadKhan2016}
  %Motivate running irregular applications (Lonestar, pannotia), discuss challenges, importance of memory divergence/coalescing, control divergence, imbalance, TLP vs ILP

  %\subsection{Graph Analytics Workloads}
  %\label{subsec:background-graph-analytics}

%   \subsection{GPU Coherence and Consistency}
%   \label{subsec:background-memory-systems}

% %   GPUs are highly parallel SIMD devices designed to execute a common program using hundreds to thousands of concurrent threads.
% %   To feed these threads, GPUs employ deeply pipelined memory hierarchies that are optimized for throughput and simplicity rather than reuse and low latency as in CPU memory hierarchies.
% %   Since the high parallelism, along with the abundant spatial locality available in modern GPU codes, is used to hide the long memory latencies, conventional GPU workloads are more sensitive to memory bandwidth than memory latency.
% %   This motivates a different cache coherence protocol than is commonly used for CPUs.
  
% %   This high parallelism is commonly used to hide memory latency in GPU codes, enabling highly efficient execution even when locality in memory accesses is limited.
% %   As a result, conventional GPU workloads are much more sensitive to memory bandwidth than memory latency, and this motivates a different coherence protocol than is commonly used for CPUs.
% %   GPU caches are therefore optimized for simplicity and throughput rather than reuse and low latency.

%   GPUs typically use simple, software-driven coherence protocols that rely on data-race freedom and assume synchronization happens infrequently and at a coarse granularity~\cite{SinclairAlsop2015}.
% %   Instead of requesting read or write permission from the last-level cache~(LLC) on a cache miss,
%   At paired synchronization reads, GPUs will self-invalidate the entire cache, and at paired synchronization writes, GPUs will write through (flush) all dirty data to the shared last level cache. 
%   Moreover, GPUs require all atomic accesses to execute at the LLC.
% %%  At synchronization points (e.g., kernel boundaries, atomic accesses, and memory fences), GPUs self-invalidate all valid data and write through (flush) all dirty data to ensure the cache does not contain stale data after the synchronization point.
% %   These flush and invalidate operations are performed in bulk across the entire cache, and in modern GPU consistency models they are triggered at synchronization points; e.g., kernel boundaries, atomic accesses, and memory fences.
%   With this coherence policy, a GPU system can offer sequentially consistent execution for any program that is data-race free.
% %   i.e., conflicting accesses in different threads which are not ordered by synchronization.
%   We refer to this coherence protocol as GPU coherence and this consistency model as DRF0 (data-race-free 0).
% %   sequential consistency for data race-free~(SC for DRF), herein referred to as DRF0.
% In DRF0, all atomic accesses are treated as paired synchronization points~\cite{AdveHill1990}.
  
%   While GPU coherence is simple, low overhead, and performs well for traditional GPU workloads, 
%   %frequent flush/invalidate operations can dramatically degrade cache efficiency. Therefore, 
%   it is inefficient for workloads that have frequent synchronization accesses.
%   Recent work has addressed this inefficiency by introducing new consistency models and coherence protocols.
% %   either by reducing the cost of flush/invalidate operations~\cite{SinclairAlsop2015}, identifying when synchronization is between threads which share a cache~\cite{HowerHechtman2014,AlsopOrr2016}, or identifying synchronization accesses where ordering constraints are not necessary for correct operation~\cite{GasterHower2015,SinclairAlsop2017}.
%   In this work, we consider the two innovations most relevant to graph algorithms: DeNovo coherence and optimized memory consistency models for heterogeneous systems.

%   Recent work has shown that DeNovo coherence
%   %although originally proposed as a simple, scalable, and efficient protocol for multi-core CPUs~\cite{ChoiKomuravelli2011,KomuravelliAdve2015, SungKomuravelli2013, SungAdve2015}, 
%   provides high performance for a wide variety of applications in heterogeneous systems~\cite{SinclairAlsop2015, AlsopSinclair2018}.
%   %offer improved reuse for workloads with fine-grained synchronization~\cite{SinclairAlsop2015}.
%   By obtaining exclusive ownership for written data and atomic accesses, data accesses don't have be invalidated or flushed for owned data and atomics can take place locally. 
%   This significantly reduces the overhead of synchronization accesses and 
%   improves reuse of written data and atomics 
%   %DeNovo achieves this by obtaining exclusive ownership for written data and atomic accesses.
%   %%Since owned data does not need to be invalidated or flushed, DeNovo makes synchronization cheaper and improves reuse 
%   while still avoiding the %throughput-limiting 
%   overheads of writer-initiated invalidations.
  
%   Recent work on memory consistency models for heterogeneous systems relaxes some of DRF0's more conservative ordering constraints.  
%   These optimizations allows programmers to specify which synchronization accesses can be relaxed and do not need to enforce DRF0's ordering constraints~\cite{GasterHower2015}, while retaining SC-centric semantics~\cite{SinclairAlsop2017}.
%   Different levels of relaxation (memory consistency models) can improve GPU performance in different ways.
%   Data-race-free-1, or DRF1~\cite{AdveHill1990}, distinguishes paired synchronization atomics from \textit{unpaired} atomics that do not order for data accesses.  
%   Unpaired atomics do not need to flush dirty data or invalidate valid data, which improves performance without affecting the DRF guarantees of DRF0.
%   Finally, data-race-free-relaxed, or DRFrlx~\cite{SinclairAlsop2017}, examined how relaxed atomics~\cite{BoehmAdve2008} were being used in practice, and showed how to extend DRF1 to provide SC or SC-centric semantics for these use cases.
%   These new categories of relaxed atomics can be reordered with both data accesses and other atomics, which reduces the need for expensive flushing and invalidating of caches and increases the amount of memory-level parallelism (MLP).
  %%allows complete reordering of data and synchronization accesses with each other
%   further relaxes the ordering constraints between atomic accesses
  %%within a thread, enabling improved memory-level parallelism~(MLP). 
  %%Unfortunately, the memory consistency semantics for fully relaxed atomics are still an open problem~\cite{SinclairAlsop2017}. For example, C++ does not provide usable semantics for these; recent work on DRFrlx has shown usable semantics for a subset of use cases~\cite{SinclairAlsop2017}. 
  %Thus, the choice of DRF1 vs.\ DRFrlx imposes a performance vs.\ programmability tradeoff.
  
  %Tightly-coupled CPU-GPU systems with unified memory address spaces and shared coherent caches may address the limitations of GPU applications with regard to irregular memory accesses and inefficient fine-grained synchronization.
  %A unified and coherent address space allows CPU and GPU cores to efficiently communicate data without the need for explicit and high-overhead data copying done in software.
  %Under such a system, using synchronization may become profitable for a larger class of applications and algorithms, if the cost of using hardware-supported atomics for both communication and synchronization is sufficiently cheap.

  %Recent work has shown that a simple coherence protocol~(DeNovo), when paired with a sequential consistency for data-race-free~(SC-for-DRF) memory model,
  %can provide dramatic improvements in fine-grained synchronization performance over traditional GPU coherence systems, and for a variety of synchronization primitives and patterns~\cite{SinclairAlsop2015}.
  %Improved synchronization efficiency is accomplished by allowing cores to obtain ownership for dirty data and synchronization variables, enabling the working set of an application to remain locally cached across synchronization boundaries.
  %This is in contrast to traditional GPU coherence schemes, which must flush all data to lower levels of the memory hierarchy at all synchronization boundaries.

  %Other works~\cite{orr:rsp} have used similar concepts with more complex consistency models, specifically heterogeneous-race-free~(HRF), to provide cheap fine-grained synchronization for work-stealing applications from the Pannotia GPU benchmark suite~\cite{che:pannotia}.
  %This work achieves improved fine-grained synchronization efficiency by optimistically keeping synchronization variables coherent at higher levels cache hierarchy, thus filtering unnecessary network traffic, until synchronization must be promoted to lower levels of the cache hierarchy.
  %Finally, works such as Lazy Release Consistency for GPUs~\cite{alsop:hlrc}, combines some of the ideas from both works to allow registration of only atomic synchronization variables with a DRF memory model, and delaying the coherence traffic for these atomic variables until they are read by remote processors; high performance for applications with dynamic atomic sharing patterns, including work-stealing graph algorithms, is achieved.

  %Ongoing work from Professor Sarita Adve's research group is geared towards exploiting the advantages of the DRF memory model and DeNovo coherence protocol for work-stealing, irregular graph applications.
  %DeNovo currently provides the unique advantage for tightly-coupled CPU-GPU systems of allowing the working set of applications with fine-grained synchronization~(via hardware atomics) to remain in the highest levels of the cache hierarchy---across synchronization boundaries, so long as the data is not to be registered for ownership by remote processors for some time.
  %Producer-consumer relationships for work queues residing in cache of the same core can exploit cheap communication and fine-grained synchronization for both data and atomic variables, even in the otherwise expensive-but-infrequent task stealing case.
  %When combined with the benefits of work-stealing on processor utilization~(i.e. rebalancing imbalanced workloads), DeNovo+DRF is uniquely poised to enable continued parallel performance scaling of work-stealing graph applications on GPUs.
  %Furthermore, the DRF model provides ease of programmability and analysis of algorithmic complexity because all data accesses, excluding accesses to atomic synchronization variables, are guaranteed to be race-free.

  %\section{Synchronization in Graph Analytics}

% \input{examples/push-pull.tex}

==> backup.tex <==
  \subsection{GPU Coherence and Consistency}
  \label{subsec:background-memory-systems}

%   GPUs are highly parallel SIMD devices designed to execute a common program using hundreds to thousands of concurrent threads.
%   To feed these threads, GPUs employ deeply pipelined memory hierarchies that are optimized for throughput and simplicity rather than reuse and low latency as in CPU memory hierarchies.
%   Since the high parallelism, along with the abundant spatial locality available in modern GPU codes, is used to hide the long memory latencies, conventional GPU workloads are more sensitive to memory bandwidth than memory latency.
%   This motivates a different cache coherence protocol than is commonly used for CPUs.
  
%   This high parallelism is commonly used to hide memory latency in GPU codes, enabling highly efficient execution even when locality in memory accesses is limited.
%   As a result, conventional GPU workloads are much more sensitive to memory bandwidth than memory latency, and this motivates a different coherence protocol than is commonly used for CPUs.
%   GPU caches are therefore optimized for simplicity and throughput rather than reuse and low latency.

  GPUs typically use simple, software-driven coherence protocols that rely on data-race freedom and assume synchronization happens infrequently and at a coarse granularity~\cite{SinclairAlsop2015}.
%   Instead of requesting read or write permission from the last-level cache~(LLC) on a cache miss,
  At paired synchronization reads, GPUs will self-invalidate the entire cache, and at paired synchronization writes, GPUs will write through (flush) all dirty data to the shared last level cache. 
  Moreover, GPUs require all atomic accesses to execute at the LLC.
%%  At synchronization points (e.g., kernel boundaries, atomic accesses, and memory fences), GPUs self-invalidate all valid data and write through (flush) all dirty data to ensure the cache does not contain stale data after the synchronization point.
%   These flush and invalidate operations are performed in bulk across the entire cache, and in modern GPU consistency models they are triggered at synchronization points; e.g., kernel boundaries, atomic accesses, and memory fences.
  With this coherence policy, a GPU system can offer sequentially consistent execution for any program that is data-race free.
%   i.e., conflicting accesses in different threads which are not ordered by synchronization.
  We refer to this coherence protocol as GPU coherence and this consistency model as DRF0 (data-race-free 0).
%   sequential consistency for data race-free~(SC for DRF), herein referred to as DRF0.
In DRF0, all atomic accesses are treated as paired synchronization points~\cite{AdveHill1990}.
  
  While GPU coherence is simple, low overhead, and performs well for traditional GPU workloads, 
  %frequent flush/invalidate operations can dramatically degrade cache efficiency. Therefore, 
  it is inefficient for workloads that have frequent synchronization accesses.
  Recent work has addressed this inefficiency by introducing new consistency models and coherence protocols.
%   either by reducing the cost of flush/invalidate operations~\cite{SinclairAlsop2015}, identifying when synchronization is between threads which share a cache~\cite{HowerHechtman2014,AlsopOrr2016}, or identifying synchronization accesses where ordering constraints are not necessary for correct operation~\cite{GasterHower2015,SinclairAlsop2017}.
  In this work, we consider the two innovations most relevant to graph algorithms: DeNovo coherence and optimized memory consistency models for heterogeneous systems.

  Recent work has shown that DeNovo coherence
  %although originally proposed as a simple, scalable, and efficient protocol for multi-core CPUs~\cite{ChoiKomuravelli2011,KomuravelliAdve2015, SungKomuravelli2013, SungAdve2015}, 
  provides high performance for a wide variety of applications in heterogeneous systems~\cite{SinclairAlsop2015, AlsopSinclair2018}.
  %offer improved reuse for workloads with fine-grained synchronization~\cite{SinclairAlsop2015}.
  By obtaining exclusive ownership for written data and atomic accesses, data accesses don't have be invalidated or flushed for owned data and atomics can take place locally. 
  This significantly reduces the overhead of synchronization accesses and 
  improves reuse of written data and atomics 
  %DeNovo achieves this by obtaining exclusive ownership for written data and atomic accesses.
  %%Since owned data does not need to be invalidated or flushed, DeNovo makes synchronization cheaper and improves reuse 
  while still avoiding the %throughput-limiting 
  overheads of writer-initiated invalidations.
  
  Recent work on memory consistency models for heterogeneous systems relaxes some of DRF0's more conservative ordering constraints.  
  These optimizations allows programmers to specify which synchronization accesses can be relaxed and do not need to enforce DRF0's ordering constraints~\cite{GasterHower2015}, while retaining SC-centric semantics~\cite{SinclairAlsop2017}.
  Different levels of relaxation (memory consistency models) can improve GPU performance in different ways.
  Data-race-free-1, or DRF1~\cite{AdveHill1990}, distinguishes paired synchronization atomics from \textit{unpaired} atomics that do not order for data accesses.  
  Unpaired atomics do not need to flush dirty data or invalidate valid data, which improves performance without affecting the DRF guarantees of DRF0.
  Finally, data-race-free-relaxed, or DRFrlx~\cite{SinclairAlsop2017}, examined how relaxed atomics~\cite{BoehmAdve2008} were being used in practice, and showed how to extend DRF1 to provide SC or SC-centric semantics for these use cases.
  These new categories of relaxed atomics can be reordered with both data accesses and other atomics, which reduces the need for expensive flushing and invalidating of caches and increases the amount of memory-level parallelism (MLP).
  %%allows complete reordering of data and synchronization accesses with each other
%   further relaxes the ordering constraints between atomic accesses
  %%within a thread, enabling improved memory-level parallelism~(MLP). 
  %%Unfortunately, the memory consistency semantics for fully relaxed atomics are still an open problem~\cite{SinclairAlsop2017}. For example, C++ does not provide usable semantics for these; recent work on DRFrlx has shown usable semantics for a subset of use cases~\cite{SinclairAlsop2017}. 
  %Thus, the choice of DRF1 vs.\ DRFrlx imposes a performance vs.\ programmability tradeoff.
  
  %Tightly-coupled CPU-GPU systems with unified memory address spaces and shared coherent caches may address the limitations of GPU applications with regard to irregular memory accesses and inefficient fine-grained synchronization.
  %A unified and coherent address space allows CPU and GPU cores to efficiently communicate data without the need for explicit and high-overhead data copying done in software.
  %Under such a system, using synchronization may become profitable for a larger class of applications and algorithms, if the cost of using hardware-supported atomics for both communication and synchronization is sufficiently cheap.

  %Recent work has shown that a simple coherence protocol~(DeNovo), when paired with a sequential consistency for data-race-free~(SC-for-DRF) memory model,
  %can provide dramatic improvements in fine-grained synchronization performance over traditional GPU coherence systems, and for a variety of synchronization primitives and patterns~\cite{SinclairAlsop2015}.
  %Improved synchronization efficiency is accomplished by allowing cores to obtain ownership for dirty data and synchronization variables, enabling the working set of an application to remain locally cached across synchronization boundaries.
  %This is in contrast to traditional GPU coherence schemes, which must flush all data to lower levels of the memory hierarchy at all synchronization boundaries.

  %Other works~\cite{orr:rsp} have used similar concepts with more complex consistency models, specifically heterogeneous-race-free~(HRF), to provide cheap fine-grained synchronization for work-stealing applications from the Pannotia GPU benchmark suite~\cite{che:pannotia}.
  %This work achieves improved fine-grained synchronization efficiency by optimistically keeping synchronization variables coherent at higher levels cache hierarchy, thus filtering unnecessary network traffic, until synchronization must be promoted to lower levels of the cache hierarchy.
  %Finally, works such as Lazy Release Consistency for GPUs~\cite{alsop:hlrc}, combines some of the ideas from both works to allow registration of only atomic synchronization variables with a DRF memory model, and delaying the coherence traffic for these atomic variables until they are read by remote processors; high performance for applications with dynamic atomic sharing patterns, including work-stealing graph algorithms, is achieved.

  %Ongoing work from Professor Sarita Adve's research group is geared towards exploiting the advantages of the DRF memory model and DeNovo coherence protocol for work-stealing, irregular graph applications.
  %DeNovo currently provides the unique advantage for tightly-coupled CPU-GPU systems of allowing the working set of applications with fine-grained synchronization~(via hardware atomics) to remain in the highest levels of the cache hierarchy---across synchronization boundaries, so long as the data is not to be registered for ownership by remote processors for some time.
  %Producer-consumer relationships for work queues residing in cache of the same core can exploit cheap communication and fine-grained synchronization for both data and atomic variables, even in the otherwise expensive-but-infrequent task stealing case.
  %When combined with the benefits of work-stealing on processor utilization~(i.e. rebalancing imbalanced workloads), DeNovo+DRF is uniquely poised to enable continued parallel performance scaling of work-stealing graph applications on GPUs.
  %Furthermore, the DRF model provides ease of programmability and analysis of algorithmic complexity because all data accesses, excluding accesses to atomic synchronization variables, are guaranteed to be race-free.

  %\section{Synchronization in Graph Analytics}

\input{examples/push-pull.tex}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



As described in Section IV-A, the structure of input graphs affects  both  the working-set  size  and  access  patterns  of  a workload. This paper calculates reasonable values for these properties statically using the CSR data as retrieved.
  There are times when our static metrics do not perfectly reflect the reality of the workload (see Section~\ref{sec:results}) but ultimately result in similar performance to optimal.
  To ensure perfect predictions, considering the temporal variations in these attributes, run-time counters available on modern GPUs could be used.
  We also note that while there may be some correlation between these properties, that only serves to limit the design space, not invalidate it.
  The following subsections breakdown how we can anticipate and specialize based on the effects caused by these properties on communication (summarized by Table II)

  %\input{tables/gs-ccc.tex}
  %\input{tables/aaa-ccc.tex}

  %\vspace{2.0cm}
  %\vspace{-0.05in}
  \subsubsection{Volume}
  \label{subsubsec:taxonomy-volume}

  The volume of data that is accessed is considered the working set size of the application, which is directly related to the size of the input graph and the workload's access patterns.
  For some algorithms, auxiliary structures which scale with the number of vertices and edges add to the size of the working set (e.g.,\ a color array for graph coloring).
  The volume of a workload is thus a function of the vertices and edges in the graph, and its effect on communication is a function of access patterns performed by the hardware.
  Although volume can also depend on the frontier size of a given iteration, the frontier size is dependent on dynamic behavior of the workload, which is difficult to compute statically.
  
  As a proxy for the working set size of a core, we compute the volume per core as an average distribution of the graph over all cores:
  \begin{equation}
      Volume(G) =
      \frac{|V(G)| + |E(G)|}{|SM|} \,.
      \label{eqn:vol}
  \end{equation}
  In Equation~\ref{eqn:vol}, $G$ is the input graph, $V$ and $E$ are functions that return the vertex and edge sets respectively, and $|SM|$ is the number of GPU cores available.
  The $Volume$ metric thus gives a value proportional to the average working set size to be touched by each GPU core.
  To anticipate whether this volume is high or low, we compare the volume of data to the available L1 and L2 resources that can be dedicated to each core during full utilization of the GPU.
  If the volume can roughly fit in each core's dedicated L1 data cache, then the volume is low.
  If the volume can fit within a core's allocation of the L2 cache~(assuming an even partitioning across cores), then the volume is medium.
  Otherwise, the volume is high.

    With medium or high volume, we expect that the workload is touching a large enough quantity of data that it limits reuse in the cache.  As a result, we generally want to maximize the amount of memory level parallelism by using DRFrlx.
    There are exceptions to this rule that will be discussed in Section~\ref{subsec:optimization-flow}.
    We also reason that volume plays a role in determining if a push or pull implementation is preferred.
    Since pull typically brings in more data into the cache, it is only preferred if the volume is low or medium.

    \subsubsection{Reuse}
    \label{subsubsec:optimization-locality}
    
    \input{figures-v6/tax-locality.tex}
    \input{examples/stats_equations.tex}

    To drive our specialization model, we need to anticipate how much intra-thread-block data reuse can be exploited in our graph workloads based on vertex connectivity.
    Figure~\ref{fig:tax-locality} depicts connectivity attributes we use that describe the potential for reuse.
    Our heuristics assume directed, symmetric graphs to match the universal input format we have for our workloads;
    however, they could be extended to express reuse for directed, non-symmetric graphs.
%     \sva{do you really cover spatial locality here?}
    
    Figure~\ref{subfig:anl} depicts the simplest case where neighbors in the graph are in the same thread block~(\textit{local neighbors}, see Equation~\ref{eqn:an-l}).
    %Such vertices are scheduled concurrently~(by thread block), and may exploit spatial locality for reads, and temporal locality for updates between them.
    Such vertices are scheduled concurrently~(by thread block), and may exploit data reuse on reads and updates to shared structures.
    
    On the other hand, Figure~\ref{subfig:anr} depicts the scenario where neighbors are placed in different thread blocks~(\textit{remote neighbors}, see Equation~\ref{eqn:an-r}).
    Achieving reuse for updates through these edges would be less likely and heavily schedule-dependent.
    We introduce the $Reuse$ metric~(Equation~\ref{eqn:loc}), combining Equations~\ref{eqn:an-l} and~\ref{eqn:an-r}.
    %To combine Equations~\ref{eqn:an-l} and~\ref{eqn:an-r} to produce an overall metric for locality, we introduce the $Locality$ metric~(Equation~\ref{eqn:loc}).
    Observe that the $AN_L$ and $AN_R$ heuristics sum to the average degree of the graph, each considering the disjoint subsets of local edges and remote edges, respectively.
    %Thus, the sum of $AN_L$ and $AN_R$ is equal to the average degree of a graph since local edges and remote edges are in disjoint sets.
    We subtract these values and normalize to the average degree of the whole graph, resulting in a term~(seen in Equation~\ref{eqn:loc}) that ranges from -1 to 1 that shows how heavily edges are skewed towards remote connectivity and local connectivity, respectively.
    As a last step, we perform some arithmetic to transform the range of the final value of $Reuse$ to a more intuitive range of 0 to 1, where 0 indicates low potential for reuse and 1 indicates high potential for reuse.
% Therefore, the result produced by the $Locality$ function where 0 indicates poor locality and 1 indicates good locality.

    $Reuse$ on its own is not sufficient to result in any optimizations choices.
    Section~\ref{subsec:optimization-flow} comments on the interactions between the $Reuse$ metric and other graph structures and algorithmic properties.

    \subsubsection{Imbalance}
    \label{subsubsec:optimization-imbalance}
    
    Beyond anticipating volume and reuse for specialization of communication, we also need to understand implications of workload imbalance.
    Imbalance of a workload is affected by the degree distribution of the graph.
    Disproportionate work allocation across the warps of a thread block (via co-scheduling high degree vertices) can cause scenarios where most of the block's warps have completed, but a small number of warps continue to process large degree vertices.
    Since each GPU core has a limited number of thread blocks that can be scheduled, long running warps in these imbalanced thread block limit the pool of warps able to be scheduled for a core.
    
    First, to compute the magnitude of imbalance, we classify warps in a thread block which contribute to high imbalance in that thread block.
    This classification is done by clustering warps in a thread block by the max degree processed by those warps.
    We accomplish this clustering via the k-means clustering algorithm, such that we search the warp for two clusters: low max degree and high max degree.
    If the difference of the final centroid's values is larger than some threshold, the thread block is considered imbalanced.
    The graph balance metric is computed to be the ratio of imbalanced thread blocks to total thread blocks~(a value from 0 to 1, inclusive).
    The larger this value, the more the imbalance is present in the graph.
    Thus imbalance is measured as follows:
    \begin{equation}
        Imbalance(G) =
        \frac{1}{|V(G)| / |TB|} \left( \sum\limits_{tb}^{TB(G)} marked(tb) \right) \,.
        \label{eqn:imb}
    \end{equation}
    In Equation~\ref{eqn:imb}, $G$ is the input graph, $V$ returns the set of vertices, $TB$ is the set of thread blocks, and $marked$ is a binary function which evaluates to 1 when our k-means algorithm determines that the given thread block is imbalanced, and 0 otherwise.

    We make no assumptions about the ordering of our graphs (i.e.,\ we do not assume a highest degree vertex ordering) so this computation must be performed for all warps.
    Further, it is not sufficient to observe a large different between average degree and max degree.
    If there is only one long-running imbalanced warp, we would only see a few (i.e.,\ 1-16) under-utilized threads.
    These long-running threads with lots of edges to process benefit greatly by allowing atomic operations to each of their neighbors to be overlapped.
    For this reason we opt for DRFrlx.
    This improves the throughput of long-running threads, decreasing run-time and increasing overall GPU utilization.
    $Imbalance$'s interactions with other properties will be discussed further in Section~\ref{subsec:optimization-flow}.
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \subsection{Algorithmic Properties}
  \label{subsec:optimization-ap}

  As described in Section~\ref{subsec:taxonomy-ap}, algorithmic properties influence the data access patterns of a graph workload.
  The following subsections describe how we can anticipate and optimize for the effects caused by these properties on communication.
  The algorithms studied in this paper largely follow the 1V1T programming paradigm, the exception being CC in which threads determine at run-time whether or not an update will be propagated (i.e.,\ NVNT).
  Table~\ref{tbl:aaa-ccc} summarizes the specialization decisions motivated by this section.
  These decisions are arrived at by analyzing each algorithms' code~(e.g., Figure~\ref{alg:push-pull}).
  
  % \sva{Need to clean up the traversal description to ensure this is true.}
%\vspace{-0.05in}

  \subsubsection{Algorithmic Traversal}
  \label{subsec:optimization-at}

  As described in Section~\ref{subsec:taxonomy-at}, algorithmic traversal determines where updates propagate to throughout the lifetime of the workload.
  % \sva{URGENT: Does the previous have to be true? it is true for cca, but in general?}
  When the algorithmic traversal of the workload is static, updates always flow between neighboring nodes in the graph~(in a vertex-centric manner).
  In this scenario, the choice of whether to use a push or pull algorithm implementation remains open~(i.e., a choice between the two kernels in Figure~\ref{alg:push-pull}).
  %Therefore, for static algorithmic traversal, we specialize using the algorithmic control, algorithmic information, and graph structure of the workload.

  For algorithms where the traversal depends on dynamically computed properties of the workload, pull and push reads or updates may race to these properties.
  Because of the racy nature of these reads and updates, DRF algorithms with dynamic algorithmic traversal require the use of fine-grained synchronization for both pulls and pushes; i.e., a non-racy pull implementation is not possible.
  Therefore, for dynamic traversal algorithms, we always specialize assuming fine-grained synchronization.%, which also interact with the coherence and consistency dimensions of the implementation design space.

  For dynamic traversal workloads, the amount of racy accesses over the lifetime of the workload over change over time.
  Some of these algorithms have a traversal which \textit{constricts} the number of possible racing accesses over time.
  This can occur when a deceasing number of worker threads process an also decreasing amount of data---this can be reflected by a decreasing number of incident dynamic edges~(and, therefore racy updates) per vertex.
  %Some algorithms can even exhibit both effects.
  In these scenarios, we can anticipate that a reduction in likelihood of racy accesses competing for the same data.
  This paired with a reduction in data volume leads us to anticipate data reuse.
  Therefore, we specialize for reuse by using DeNovo coherence, allowing racy accesses to receive ownership at the L1.
  
  Other dynamic traversal algorithms can exist where the number of racy accesses to the same data does \textit{not constrict}.
  %\footnote{None of our applications showed this phenomenon but we include it here for completeness.}
  This can occur if the number of worker threads does not decrease over time, but the working dataset converges to an increasingly smaller size.
  We argue that in such a case DeNovo is still preferable.  As the dataset converges, each atomic access bringing data into the L1 will serve an increasing number of requests from threads in that SM.  We believe that this more than offsets the cost of ping-ponging.
  This is compared to GPU coherence which will serialize requests at the L2.  L2 atomics to the same address must be serialized to account for ordering requirements; there is no distinction made between atomic requests from the same thread or different different threads within a warp as it would be infeasible to include something like threadID in the MSHR.
  Such a distinction is not needed when working with in-order networks, but that solution will not scale as GPUs increase core-counts and is not modeled in our simulator as a result.

  As mentioned, dynamic traversal workloads require extensive use of fine-grained synchronization.
  Moreover, these algorithms require the values returned by these racy accesses in order to determine the traversal's control flow.
  Since the values for these racy accesses are being read, diligent reasoning by the programmer should be used to determine whether these racy accesses can be relaxed using DRFrlx according to the specification described in~\cite{SinclairAlsop2017}.
  Additionally, a consequence of reading the values returned by racy accesses for control flow is that a thread must wait for the values to proceed computation, limiting the impact of atomic relaxation on performance.
  Therefore, specialize for a consistency model that offers ease of programmability~(DRF1) without considerable loss in performance.

  \subsubsection{Algorithmic Control}
  \label{subsec:optimization-ac}

  As described in Section~\ref{subsec:taxonomy-ac}, algorithmic control determines the control flow of a program~(i.e., when updates should propagate across an edge).
  The control flow, in turn, dictates the amount of work and communication that is performed, implicitly affecting the working set size.

  When algorithmic control is asymmetric with regard to predicate checks of the source and target nodes, we should to elide as much control and computation as possible~(Section~\ref{subsec:taxonomy-ac}).
  To do so, we specialize for the push/pull implementation which nests the least amount of control flow in the inner loop of an edge traversal~(Figure~\ref{alg:push-pull}).
  If more work is elided at the source, we prefer a push implementation; if more work is elided at the target, we have an inclination towards a pull implemented.
  Note that specializing for racy updates requires the use of fine-grained synchronization~(RMWs) in the code~(line 8 of the push kernel in Figure~\ref{alg:push-pull}).
  
  If the algorithmic control is symmetric between a push and pull kernel for the algorithm, or if the algorithm does not have any predicate checks in either loop body, we do not have the opportunity to specialize based on the control flow.
  
  %\vspace{-0.05in}
  \subsubsection{Algorithmic Information}
  \label{subsec:optimization-ai}

  As described in Section~\ref{subsec:taxonomy-ai}, algorithmic information influences the working set size of the workload.
  By specializing for working set size, we aim to minimize the amount of communication done by each thread.

  If the algorithm has asymmetry in the number of loads between a push and pull kernel, we specialize for the push or pull design which hoists the largest amount of variables accessed into the outer loop~(see $s$ and $t$ loop body positions in Figure~\ref{alg:push-pull}).
  Again, if the application hoists more loads at the source, we prefer for push; if more loads are hoisted at the target, there is a predisposition pull.
  Doing so amortizes the cost of accessing the outer loop vertex's property by performing them once, instead of once per incident edge. 
  
  When there is symmetry in algorithmic information, no specialization for raciness hoists more accesses.

==> figures-v6/at.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[keepaspectratio,width=0.6\columnwidth]{figures-v6/at-fig-crop.pdf}%
  \captionsetup{font=footnotesize}
  \caption{Static and dynamic algorithmic traversals. Static causes updates to flow through actual neighboring nodes in the graph~(via edges in solid blue). Dynamic  allows updates to flow across the graph via indirect links between nodes that are not neighbors~(via the edge in dotted gray).}%
  %\belowcaptionskip
  \label{fig:at}%
\end{figure}%


==> figures-v6/conflicts-flow-chart.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[keepaspectratio,height=2.5in]{figures-v6/aaa-flow-chart.png}%
  \caption{Methodology for navigating through algorithmic properties~(Traversal, Control, and Information) when choosing system implementation designs.}
  %\includegraphics[keepaspectratio,height=2.5in]{figures-v6/conflicts-flow-chart.png}%
  %\caption{Steps involved in a workload-driven design for the choice of C vs.\ N. The flow chart starts by considering the AT property of the workload, followed by the AC, and then the AI. This order is the priority of the properties' effect on performance. The sinks of the flowchart indicate if the optimal design space for the workload has narrowed and how.}%
  \label{fig:conflicts-flow-chart}%
\end{figure}%


==> figures-v6/gs-flow-chart.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[keepaspectratio,height=2.5in]{figures-v6/gs-flow-chart.png}%
  \caption{Methodology for navigating through graph structure properties~(volume, locality, and imbalance) when choosing system implementation designs.}
  %\includegraphics[keepaspectratio,height=2.5in]{figures-v6/conflicts-flow-chart.png}%
  %\caption{Steps involved in a workload-driven design for the choice of C vs.\ N. The flow chart starts by considering the AT property of the workload, followed by the AC, and then the AI. This order is the priority of the properties' effect on performance. The sinks of the flowchart indicate if the optimal design space for the workload has narrowed and how.}%
  \label{fig:gs-flow-chart}%
\end{figure}%


==> qualitative.tex <==
\section{Workload-Driven Specialization}
\label{sec:optimization}

% In Section~\ref{sec:taxonomy}, we introduced four properties of graph analytics workloads that interact with the communication design space.
This section introduces a model that establishes how to specialize the raciness of the algorithm and the coherence and consistency of the memory system based on the application and input-dependent features introduced in our taxonomy~(see Section~\ref{sec:taxonomy}).
We note that previous work, such as \cite{WangPan2017}, has studied push vs.\ pull implementations of algorithms for GPUs; that work focuses on conventional GPUs and does not consider the effects of varying coherence or consistency.
Section~\ref{subsec:optimization-gs} describes how to specialize based on the input graph structure.
Section~\ref{subsec:optimization-ap} describes how to specialize based on the algorithmic properties.
Tables~\ref{tbl:gs-ccc} and~\ref{tbl:aaa-ccc} summarize the specializations recommended by both these sections, respectively.
Finally, Section~\ref{subsec:optimization-nav} describes a structured method to use our model to specialize using information about both the graph and the algorithm in unison.
%that links each workload property introduced in Section~\ref{sec:taxonomy} with each communication dimension discussed in Section~\ref{sec:comm-design-space}.

  \subsection{Graph Structure}
  \label{subsec:optimization-gs}

  %\input{tables/gs-ccc.tex}
  \input{tables/aaa-ccc.tex}
  
  As described in Section~\ref{subsec:taxonomy-gs}, the structure of input graphs affects both the working-set size and access patterns of a workload.
  The salient aspects of graph structure as it impacts \hl{communication} \whd{Do we still want to call this communication} are the \emph{volume} and \emph{locality} of accessed data, and the work \emph{imbalance} per work item.
  This paper calculates reasonable values for these properties statically using the CSR data as retrieved.  There are times when our static metrics do not perfectly reflect the reality of the workload (see Section~\ref{sec:results}) but ultimately result in similar performance to optimal.
  To ensure perfect predictions, considering the temporal variations in these attributes, run-time counters available on modern GPUs could be used.
  We also note that while there may be some correlation between these properties, that only serves to limit the design space, not invalidate it.
  The following subsections breakdown how we can anticipate and specialize based on the effects caused by these properties on communication~(summarized by Table~\ref{tbl:gs-ccc}).

  %\vspace{2.0cm}
  %\vspace{-0.05in}
  \subsubsection{Volume}
  \label{subsubsec:optimization-volume}

    \input{figures-v6/tax-locality.tex}
    
    \input{examples/stats_equations.tex}

  The volume of data that is accessed as it resides in cache is considered the working set size of the application, which is directly related to the size of the input graph and the workload's access patterns.
  For some algorithms, auxiliary structures which scale with the number of vertices and edges add to the volume of the working set (e.g.,\ a color array for graph coloring).
  The volume of a workload is thus a function of the vertices and edges in the graph, and its effect on communication is a function of access patterns performed by the hardware.
  Although volume can also depend on the frontier size of a given iteration, the frontier size is dependent on dynamic behavior of the workload, which is difficult to compute statically.
  
  As a proxy for the working set size of a core, we compute the volume per core as an average distribution of the graph over all cores:
  \begin{equation}
      Volume(G) =
      \frac{|V(G)| + |E(G)|}{|SM|} \,.
      \label{eqn:vol}
  \end{equation}
  In Equation~\ref{eqn:vol}, $G$ is the input graph, $V$ and $E$ are functions that return the vertex and edge sets respectively, and $|SM|$ is the number of GPU cores available.
  The $Volume$ metric thus gives a value proportional to the average working set size to be touched by each GPU core.
  To anticipate whether this volume is high or low, we compare the volume of data to the available L1 and L2 resources that can be dedicated to each core during full utilization of the GPU.
  If the volume can roughly fit in each core's dedicated L1 data cache, then the volume is low.
  If the volume can fit within a core's allocation of the L2 cache~(assuming an even partitioning across cores), then the volume is medium.
  Otherwise, the volume is high.

  %On a per thread basis, we can compute the number of vertices to be processed and the number of updates the thread will perform.
  %Thread volume can be summarized based on
  %by computing the average and maximum degrees (volume upper bound) of the vertices assigned to each thread.

  For low volume inputs when using racy updates, we should opt for configurations with ownership for atomic operations~(DeNovo coherence) to increase potential for intra-kernel reuse.
  For low volume inputs when using non-racy updates for DRF programs, intra-kernel reuse is comparable for the updates for both DeNovo and GPU coherence because both protocols perform updates to data at the L1 once the valid brought into the cache.
  Unlike GPU coherence, DeNovo also offers potential inter-kernel reuse when an input is low volume, because DeNovo allows registration of ownership for both data and atomics which will remain in the L1 cache across kernel synchronization boundaries, given L1 capacity is not an issue.
  Therefore, for low volume inputs, we can safely specialize for DeNovo.
  %WHD: We also want to consider low volume will give us intra-thread and possibly inter-kernel reuse.  When Gio say's intra-kernel, does he mean intra-thread? Or does he mean that if the volume is low, it's just statistically likely that we'll get some reuse.
  
  High volume inputs can cause reuse to be difficult to exploit due to L1 cache pollution.
  Pollution leading to low reuse at the L1 can occur when the working set for updates evicts data required for graph traversal, for example.
%   Keeping data around for address generation is a first-order concern because these computations are on the critical path for sparse, irregular workloads.
  Thus, for these inputs, we can specialize to perform updates in-memory~(push + GPU coherence) to alleviate pollution.
  Finally, for medium volume inputs, where it is less clear whether cache pollution at the L1 will be problematic for performance, we conservatively specialize for GPU coherence (i.e.\ the simpler option) as a middle ground between the low and high volume input scenarios.
%   to avoid unnecessary eviction of critical path data~(for address generation).
  
  In the consistency dimension, optimization for volume is difficult because performance depends on dynamic access patterns of the workload.
  If hardware resources which support MLP~(MSHRs at the L1) are saturated by the working set, then DRF1 should perform similarly to DRFrlx.
  In this case, we can opt for DRF1 due to ease of programmability.
  If these resources are not saturated, and the working set is large enough, then DRFrlx should offer improved performance at the cost of programmability.
  %\whd{This would be a good place to comment on a future dynamic runtime system (because these are heuristics and although we chose to keep to static analysis for simplicity, that shouldn't be a limiting factor.)}
  %\mh{In theory this would be good to say, but you'd have to phrase this \emph{very} carefully.}
  However, given that the utilization of these resources is difficult to measure statically, we do not opt for either consistency model based on volume.
  
  \textit{Applying the Model}---By using simple features of the graph~(number of vertices and edges) and the hardware available~(cache sizes and number of cores), the volume metric used~(Equation~\ref{eqn:vol}) can be easily computed at compile-time, load-time, or run-time.
%   \textit{Implications for Run-times}---The methodology described here only requires knowing simple features of the graph~(number of vertices and edges) and the hardware available~(cache sizes and number of cores), and the volume metric used~(Equation~\ref{eqn:vol}) is inexpensive to compute.
%   This portion of the workload-driven design can be computed at any stage -- compile-time, load-time, or run-time -- of the design where the graph and hardware metadata is made available.
%   This could occur either statically at either compile-time, load-time, or run-time.
  Therefore, a flexible software-hardware interface can be used to specialize the system as soon as the required metadata is known.

  %Furthermore, since MLP is abundant due to the large number of accesses, relaxed memory ordering~(R) is not as critical.
  %Finally, the raw volume of data accessed alone does not affect the optimality of conflicts versus no conflicts.

%   \note{The solution to our owned atomics latency bug determines whether we care about optimization for 1+L2 vs R+OA here depending on expected cache utilization/locality.}

  %By optimizing for the workload's AIS, we aim to understand the concurrency that may introduce data-races which interface consistency model and coherence protocol.
  %We also aim to optimize for the working dataset size as affected by the concurrency in the program and the coherence protocol employed.

  %For algorithms with an AIS resembling indirect pointer jumping, the concurrency in the program is dictated by its traversal through the dynamic structure of the graph.
  %In other words, the propensity for the workload to have data-races is non-deterministic and fixed by the structure of the algorithm.
  %Therefore, the AIS has a significant impact of the concurrency of the application, but this dimension of communication is no longer a design space that can be optimized.
  %However, the presence of data-races means that the choice of consistency model and coherence protocol has a large impact on performance.

  %For algorithms with an AIS where information flows through edge-propagated updates, the concurrency in the program remains a design space for optimization.
  %Given this option, we use the algorithm's other properties and the input structure to determine the optimal communication design for the three dimensions.

  %When considering the affect of input structure on communication, we must remember the impact of data-races.
  %For algorithms with indirect pointer jumping, data-races will arise from emergent properties of the graph that are computed dynamically.
  %For algorithms with edge-propagated updates, data-races will be present as a function of the connectivity between vertices~(i.e., their degrees).
  %For designs where the input structure and concurrency introduce many races in the workload, the AIS exacerbates the performance impact of the consistency model.
  %The relaxation of fine-grained synchronization becomes a first-order optimization concern.

  %Beyond considering concurrency and consistency, high connectivity, whether through static or emergent structure of the graph, has performance implications on locality of shared data.
  %Therefore, once the properties and components of communication that introduce data-races have been fixed, optimality of communication through coherence becomes significant.
  % 
  %To summarize as shown in Table~\ref{tbl:aaa-ccc}, AISs have a significant impact on the concurrency of a workload and the amount of data-races as a function of the input structure.
  %Therefore, AISs have a significant impact on the entire design space of communication that we explore.

    \subsubsection{Locality}
    \label{subsubsec:optimization-locality}

    To drive our specialization model, we need to anticipate how much locality can be exploited in our graph workloads based on vertex connectivity.
%     \sva{There is no description of this at all. We don't even know what each equation refers to. Put some brief explanation in the caption of the figure minimally. say what the different variables are.}
    Based on the connectivity of vertices, we characterize opportunities for temporal and spatial locality of each workload.
    %For simplicity, we define these attributes using thread blocks to capture locality of co-scheduled vertices without worrying about which cores thread blocks are scheduled to.
    Figure~\ref{fig:tax-locality} depicts connectivity attributes we use that describe the potential for locality.
    Our heuristics assume directed, symmetric graphs to simplify the computation;
    however, they could be extended to express locality for directed, non-symmetric graphs.
%     \sva{do you really cover spatial locality here?}
    
    Figure~\ref{subfig:anl} depicts the simplest case where neighbors in the graph are in the same thread block~(\textit{local neighbors}, see Equation~\ref{eqn:an-l}).
    Such vertices are scheduled concurrently~(by thread block), and may exploit spatial locality for reads, and temporal locality for updates between them.
    
    On the other hand, Figure~\ref{subfig:anr} depicts the scenario where neighbors are placed in different thread blocks~(\textit{remote neighbors}, see Equation~\ref{eqn:an-r}).
    Achieving locality for updates through these edges would be less likely and heavily schedule-dependent, compared to vertices in the same thread block.
    To combine Equations~\ref{eqn:an-l} and~\ref{eqn:an-r} to produce an overall metric for locality, we introduce the $Locality$ metric~(Equation~\ref{eqn:loc}).
    Observe that the $AN_L$ and $AN_R$ heuristics compute the average degree of the graph, each considering only the subset of local edges and remote edges, respectively.
    Thus, the sum of $AN_L$ and $AN_R$ is equal to the average degree of a graph since local edges and remote edges are in disjoint sets.
    If instead we subtract these values and normalize to the average degree of the whole graph, we arrive with a term~(seen in Equation~\ref{eqn:loc}) that ranges from -1 to 1 that shows how heavily edges are skewed towards local connectivity and remote connectivity, respectively.
    As a last step, we perform some arithmetic to transform the range of the final value of $Locality$ to a more intuitive range of 0 to 1, where 0 indicates poor locality and 1 indicates good locality.
% Therefore, the result produced by the $Locality$ function where 0 indicates poor locality and 1 indicates good locality.

    %We also introduce attributes to describe locality through intermediary vertices~(\textit{second neighbors}).
    %This helps us understand temporal locality when a pair of vertices are collaboratively updating a common third node.
    %Figure~\ref{subfig:ansl}~(see Equation~\ref{eqn:asn-l}) depicts the scenario where two vertices~($s$ and $u$) in the same thread block $TB_i$ have a connection to a common vertex $t$ in some thread block $TB_j$.
    %If $s$ and $u$ process updates to $t$ in quick succession, then they are likely to exploit temporal locality.
    %We can also capture increased potential for spatial locality if vertices $s$ and $u$ are close enough in the thread block to be on the same cache line.
    %
    %Figure~\ref{subfig:ansr}~(see Equation~\ref{eqn:asn-r}) depicts the opposite scenario where vertices $s$ and $u$ are not in the same thread block, but are still both connected to $t$.
    %When this occurs, $s$ and $u$ are much less likely to exploit temporal locality.
    %Moreover, if they both request ownership in their local caches for data properties of $t$, they may contend and decrease performance of the workload.

    Locality can affect the choice of racy updates, coherence, and consistency in the system implementation design space.
%     \sva{This does not comment on the consistency model choice though it says locality affects everything.}
    For inputs where we anticipate a lot of temporal locality, we should specialize for owned atomics~(DeNovo coherence) when using racy push updates.
    As a corollary to the high volume optimization described in Section~\ref{subsubsec:optimization-volume}, DeNovo and GPU coherence exploit comparable intra-kernel temporal reuse for non-racy pull updates since they are dense and local at the L1 ~(once the valid data is brought into the cache).
    Therefore, for high locality graphs, we can safely specialize for DeNovo.
    If our inputs are anticipated to have low temporal locality, we should specialize for designs that perform racy updates in-memory~(push + GPU coherence) to avoid unnecessary evictions in the L1~(i.e., data used for graph traversal).
    % of critical data~(address generation) from the L1.

    Regarding consistency, unlike DRF0, both DRF1 and DRFrlx allow for read-modify-write atomic updates to reorder freely with respect to non-dependent data accesses without initiating L1 self-invalidations that reduce opportunities for reuse.
    As such, atomic data brought into the L1 cache can be reused within a kernel.
    Additional performance can sometimes be achieved by DRFrlx at the cost of programmability, but as described in Section~\ref{subsubsec:optimization-volume}, this is dependent on utilization of resources that offer improved MLP~(e.g., MSHRs).
    Statically predicting utilization of resources that depend on dynamic data access patterns is difficult, so we do not specialize consistency models based on locality.
    
    %In the scenario that locality for the input is low, we prefer also to use DRFrlx in order to maximize throughput of the GPU~(similar to the high volume input case described in Section~\ref{subsubsec:optimization-volume}.
    %While, relaxation of atomic updates can affect cache conflict misses~(and subsequently, locality), we don't consider these effects in the context of locality for simplicity of analysis.
    %Therefore, we don't prefer either consistency design in this work when optimizing for locality.

    %\note{Add para here for equations.}
    
    \textit{Applying the Model}---The locality metric can be computed statically to guide the choice of the best system implementation.
    Alternatively, during execution, hardware counters~(e.g., hit rate counters) can be used to capture exactly how much locality is experienced by a kernel.
    % \textit{Implications for Run-times}---The methodology described here requires enumerating how much of the connectivity of each thread block falls within that thread block, as well as knowing the average degree of the entire graph.
    % While this metric is simple to compute statically, it is a relatively expensive computation to compute at run-time because measuring the connectivity requires the same indirection of access for neighboring edges that irregular graph kernels need to perform.
    % One solution for computing the locality at run-time would be to leverage that the primary computation of most graph kernels already needs to visit the neighbors of vertices during processing.
    % Each thread block could then locally compute how many edges fall within that thread block by using a intra-thread block reduction of local edges.
    % However, this remains a non-negligible computation overhead.
    % A second solution is to directly use hardware counters~(hit rate counters) to capture exactly how much locality is experienced by a kernel.
    % Then given an iteration, the hit rate experienced could be used to forecast locality to be experienced by future iterations.
    % While using counters is a more direct measure of locality, our heuristic captures the salient structure of locality for thread blocks and can be used for our static analysis.
    When the run-time detects changes in the demands of the workload, it can leverage a system with a flexible software-hardware interface such as \cite{AlsopSinclair2018} to
    % influence the system implementation to
    specialize for improved locality in future iterations.

    \subsubsection{Imbalance}
    \label{subsubsec:optimization-imbalance}
    
    Beyond anticipating volume and locality for specialization of communication, we also need to understand implications of workload imbalance.
    Imbalance of a workload is affected by the degree distribution of the graph.
    %The thread blocks with heavy imbalance will have a larger proportion of threads processing vertices with large degrees, and subsequently warps with vertices of large degrees.
    %When thread blocks are heavily imbalanced with respect to other thread blocks due to disproportionate work allocation, these thread blocks hold up the entire GPU kernel.
    Disproportionate work allocation across the warps of a thread block can cause scenarios where most of the block's warps have completed, but a small number of warps continue to process large degree vertices.
    Since each GPU core has a limited number of thread blocks that can be scheduled, long running warps in these imbalanced thread block limit the pool of schedulable warps for the core.
    Thus, thread blocks imbalanced in this way can hamper the MLP of their cores.
    Speeding up those long running threads in the imbalanced warps by exploiting
    % more ILP~(concurrent address generations) and
    intra-thread MLP~(concurrent updates from the same vertex) can significantly reduce this critical path delay in the core~(an thus the kernel overall).
    
    First, to compute the magnitude of imbalance, we classify warps in a thread block which contribute to high imbalance in that thread block.
    This classification is done by clustering warps in a thread block by the max degree processed by those warps.
    We accomplish this clustering via the k-means clustering algorithm, such that we search for two warp clusters: low max degree and high max degree.
    If the difference of the final centroid's max degree values is larger than some threshold, then the thread block is imbalanced.
    The graph balance metric is computed to be the ratio of imbalanced thread blocks to total thread blocks~(a value from 0 to 1, inclusive).
    The larger this value, the more the imbalance is present in the graph.
    Thus imbalance is measured as follows:
    \begin{equation}
        Imbalance(G) =
        \frac{1}{|V(G)| / |TB|} \left( \sum\limits_{tb}^{TB(G)} marked(tb) \right) \,.
        \label{eqn:imb}
    \end{equation}
    In Equation~\ref{eqn:imb}, $G$ is the input graph, $V$ is the set of vertices, $TB$ is the set of thread blocks, and $marked$ is a binary function which evaluates to 1 when our k-means algorithm determines that the given thread block is imbalanced, and 0 otherwise.

    For the design space we explore, the primary way to achieve more
    % ILP and
    intra-thread MLP for long running warps is to allow the long threads in these warps to reorder
    % data accesses~(address generation) and
    updates.
    %The second way is to improve locality in the caches to ensure that accesses are satisfied quickly.
    For DRF programs, non-racy pull updates can already be reordered to this effect since the updates are normal data accesses.
    When using racy push updates, we can achieve the desired effect in an MLP-starved workload by using a relaxed consistency model~(DRFrlx).
    The ability to reorder both data or atomic accesses implies that either non-racy or racy updates could be viable for specialization.
    However, Figure~\ref{alg:push-pull} shows that non-racy pull updates must wait on sparse remote reads that are on the critical path for updates~(lines 8--10).
    Racy updates, assuming DRFrlx, can fire off updates to the memory system while moving on other updates that are only dependent on local dense reads~(lines 4 and 8).
    %Since the consistency models we explore do not interact with non-racy updates within a kernel, we can safely opt for DRFrlx when processing highly imbalanced graphs.
    Therefore for high imbalance graphs, we specialize for racy updates with DRFrlx.
    If the graph structure does not show high imbalance, the high memory throughput of GPUs is unlikely to be starved by long running threads, allowing the possibility of optimizing for programmability~(using DRF0 or DRF1) using either non-racy or racy updates.
    
    \textit{Applying the Model}---While performing k-means clustering at run-time is expensive, the salient structure of imbalance captured by our metric, warp imbalance, can be leveraged by a run-time system for dynamic specialization.  
    %\mh{If you can't cite a paper we can list the real-world occupancy and utilization counters in both NVIDIA and AMD GPUs.  NVIDIA has even more complex ones, but we don't need to worry about that rn.}
    % \textit{Implications for Run-times}---The methodology described here requires computing the k-means clustering by max warp degree of every thread block in the kernel.
    % While this computation is likely too expensive to perform at run-time, the salient structure of the imbalance captured by our metric can be leveraged by a run-time system.
    
    When GPU cores with warp imbalance are detected, run-time can configure the consistency model appropriately to speed up threads on the critical path of these warps.
    \whd{Huzi and I believe the above statement to be wrong/narrative breaking.  Given a dynamic system that is capable of DRF1 and DRFRlx, and given that we have a binary that has correctly reasoned about the relaxed atomics, why would we not always use relaxed atomics?}
    
    % A software run-time or hardware monitor can search for GPU cores that have thread blocks scheduled such that most of the warps have completed execution, but there still remains warps with large amounts of edges to process.
    % At these points in time, the run-time can take the necessary action for the consistency model in order to speed up the threads on the critical path in order to quickly free up resources occupied by those threads blocks.

  \subsection{Algorithmic Properties}
  \label{subsec:optimization-ap}

  %\input{tables/aaa-ccc.tex}

  As described in Section~\ref{subsec:taxonomy-ap}, algorithmic properties influence the data access patterns of a graph workload.
  The following subsections describe how we can anticipate and optimize for the effects caused by these properties on communication.
  The algorithms studied in this paper largely follow the 1V1T programming paradigm, the exception being CC in which threads determine at run-time whether or not an update will be propagated (i.e.,\ NVNT).
  Table~\ref{tbl:aaa-ccc} summarizes the specialization decisions motivated by this section.
  These decisions are arrived at by analyzing each algorithms' code~(e.g., Figure~\ref{alg:push-pull}).
  
  % \sva{Need to clean up the traversal description to ensure this is true.}
%\vspace{-0.05in}

  \subsubsection{Algorithmic Traversal}
  \label{subsec:optimization-at}

  As described in Section~\ref{subsec:taxonomy-at}, algorithmic traversal determines where updates propagate to throughout the lifetime of the workload.
  % \sva{URGENT: Does the previous have to be true? it is true for cca, but in general?}
  When the algorithmic traversal of the workload is static, updates always flow between neighboring nodes in the graph~(in a vertex-centric manner).
  In this scenario, the choice of whether to use racy updates or not~(via a pull kernel or a push kernel) remains open~(i.e., a choice between the two kernels in Figure~\ref{alg:push-pull}).
  Therefore, for static algorithmic traversal, we specialize using the algorithmic control, algorithmic information, and graph structure of the workload.

  For algorithms where the traversal depends on dynamically computed properties of the workload, pull and push reads or updates may race to these properties.
  Because of the racy nature of these reads and updates, DRF algorithms with dynamic algorithmic traversal require the use of fine-grained synchronization for both pulls and pushes; i.e., a non-racy pull implementation is not possible.
  \whd{We've defined racy in such a way that racy-atomics makes sense, but it was confusing to me at first glance and our reviewers.}
  Therefore, for dynamic traversal algorithms, we always specialize assuming racy atomics.%, which also interact with the coherence and consistency dimensions of the implementation design space.

  For dynamic traversal workloads, the amount of racy accesses over the lifetime of the workload over change over time.
  Some of these algorithms have a traversal which \textit{constricts} the number of possible racing accesses over time.
  This can occur when a deceasing number of worker threads process an also decreasing amount of data---this can be reflected by a decreasing number of incident dynamic edges~(and, therefore racy updates) per vertex.
  %Some algorithms can even exhibit both effects.
  In these scenarios, we can anticipate that a reduction in likelihood of racy accesses competing for the same data.
  Therefore for these workloads, we specialize for locality by using DeNovo coherence, allowing racy accesses to receive ownership at the L1.
  
%   \whd{I want to spend some time with Huzi and go over the correctness for this statement.  It makes sense on a surface level, but because of the structure of our CC implementation I want to discuss.  We do 1 loop and then a complete cleanup.  In the original code there were 3 stages so it might have been more observable, but when I looked at the atomic access information for John it wasn't clear that in our implementation we are shrinking accesses (at least at the phase granularity).}
%   \mh{We want DeNovo in \emph{any} dynamic traversal scenario. 1. If data constricts, one owned request will service a lot of people. 2. If data doesn't constrict, there is no ping-ponging. \#raced addresses will impact the benefit over GPU coherence but in general should still be a win.}
%   \mh{Counter example to above: data doesn't constrict but is also shared by everyone. This is similar to a standard static traversal so can call it a tie.}
%   \whd{i.e.\ instead of irregular accesses to neighbors, it's irregular accesses to any vertex.  Given that we aren't making any assumptions about the locality of the neighbors in the static traversal case, these act similarly given the working set is larger than the cache.}
%   \mh{Model justification: 1. In order networks are not possible in future systems. 2. DRF is desirable. 3. Real MSHRs cannot be tagged with tid. 4. Ergo, our model is the way to go.}
  
  Other dynamic traversal algorithms can exist where the number of racy accesses to the same data does \textit{not constrict}.
  %\footnote{None of our applications showed this phenomenon but we include it here for completeness.}
  This can occur if the number of worker threads does not decrease over time, but the working dataset converges to an increasingly smaller size.
  We argue that in such a case DeNovo is still preferable.  As the dataset converges, each atomic access bringing data into the L1 will serve an increasing number of requests from threads in that SM.  We believe that this more than offsets the cost of ping-ponging.
  This is compared to GPU coherence which will serialize requests at the L2.  L2 atomics to the same address must be serialized to account for ordering requirements; there is no distinction made between atomic requests from the same thread or different different threads within a warp as it would be infeasible to include something like threadID in the MSHR.
  Such a distinction is not needed when working with in-order networks, but that solution will not scale as GPUs increase core-counts and is not modeled in our simulator as a result.
  
  %Therefore, a coherence protocol registers ownership at the L1 for the contested atomic dataset can hamper performance due to ping-ponging ownership forwarding.
  %Thus, we specialize for GPU coherence to perform these racy updates directly at the L2 with a lower latency.
  
  %For these algorithms we can expect large amounts of RMWs accesses which contend in the memory system if the number of threads performing these racy updates remains constant over the workload's lifetime.
  %In this scenario, we should avoid using a coherence protocol requires bringing atomic data into the local cache~(via ownership registration) to avoid high latency ping-ponging of data~(DeNovo).
  %Therefore, we prefer to use GPU coherence for these algorithms.

  %On the other hand, if the algorithm with dynamic traversal does not experience increased contention in the memory system over the lifetime of the workload~(i.e., the working set does not constrict, or the number of active threads monotonically decreases), getting ownership for atomic data is not a performance concern.
  %Moreover, we may benefit from improved performance in the presence of temporal locality in the workload.
  %For these algorithms, we opt for using DeNovo coherence to enable ownership for atomic data.
  
  %the number of conflicts is determined by the structure of graph, the dynamic properties computed and traversed, as well as the non-deterministic resolution of conflicts which are tied to control flow.
  %However, this contention only exists if the number of threads accessing the smaller subset of data remains the same or grows.
  %For algorithms which have an increasingly smaller number of threads over time, we should optimize for locality on this small subset of data via owned atomics~(D).
  %For both cases, the presence of conflicts means that we should optimize for non-blocking atomic operations to maximally exploit the MLP available.

  As mentioned, dynamic traversal workloads require extensive use of fine-grained synchronization.
  Moreover, these algorithms require the values returned by these racy accesses in order to determine the traversal's control flow.
  Since the values for these racy accesses are being read, diligent reasoning by the programmer should be used to determine whether these racy accesses can be relaxed using DRFrlx according to the specification described in~\cite{SinclairAlsop2017}.
  Additionally, a consequence of reading the values returned by racy accesses for control flow is that a thread must wait for the values to proceed computation, limiting the impact of atomic relaxation on performance.
  Therefore, specialize for a consistency model that offers ease of programmability~(DRF1) without loss in performance.
  Still, for completeness of our evaluation, we include specialization for dynamic traversal using DRFrlx to the understand performance of these workloads.
  %Therefore, for algorithms with dynamic traversal, we conservatively prefer DRFrlx to avoid a large amount of blocking atomic throughout the traversal.

  % This design space is summarized in Table~\ref{tbl:aaa-ccc}.
%   The methodology in Section~\ref{subsec:optimization-gs} applies for static AT.\sva{the last sentence strictly doesnt make sense. what methodology? what does it mean for it to apply to static at?}

%   \note{Talk about the anomaly in using relaxed atomics in the results section.}
%\vspace{-0.05in}
  \subsubsection{Algorithmic Control}
  \label{subsec:optimization-ac}

  As described in Section~\ref{subsec:taxonomy-ac}, algorithmic control determines the control flow of a program~(i.e., when updates should propagate across an edge).
  The control flow, in turn, dictates the amount of work and communication that is performed.
%   Therefore, the effect of AC on the optimization space for communication depends on the class \sva{what is class?} of algorithm, and whether there is room to optimize for control flow.

  %For algorithms in the space of topologically-driven, vertex-centric implementation, we have two scenarios.
  %In the first scenario, the algorithm has no ACRs.
  %For these algorithms, the design space of communication should be optimized with respect to algorithm's other properties in the taxonomy, keeping in mind the coupling and prioritization the components of communication.

  When algorithmic control is asymmetric with regard to predicate checks of the source and target nodes, we should elide as much control and computation as possible~(Section~\ref{subsec:taxonomy-ac}).
  To do so, we specialize for the raciness implementation~(either push or pull) which nests the least amount of control flow in the inner loop of an edge traversal~(Figure~\ref{alg:push-pull}).
%   Note that this choice has further implications on the introduction of conflicts, \sva{what does the previous mean - dont we already describe the implications?} and subsequently, on optimization for fine-grained synchronization.\sva{why arent we describing the implications for fine grained synch here. we never talk about fine grain synch. why is this suddenly used here. i am confused.}
  Note that specializing for racy updates requires the use of fine-grained synchronization~(RMWs) in the code~(line 8 of the push kernel in Figure~\ref{alg:push-pull}).
  
  If the algorithmic control is symmetric between a push and pull kernel for the algorithm, or if the algorithm does not have any predicate checks in either loop body, we do not have the opportunity to specialize based on the control flow.
  Thus for symmetric control, graph structure and the other algorithmic properties will factor into specialization decisions.
  %In this scenario, we do not make a recommendation for any of the implementation dimensions.
  % This design space is summarized in Table~\ref{tbl:aaa-ccc}.

  %We must then consider the symmetry of control flow requirements~(depicted in Figure~\ref{fig:aaa}) and their affect on communication.
  %In the case that the ACRs are symmetric~(in performance overhead) for both sides of an edge, we optimize for communication in a similar fashion as for algorithms with no ACRs.
  %If the ACRs are asymmetric on either side of an edge, we should optimize control flow such that we satisfy the most ACRs earlier in the control of the workload.
  %This allows us to elide as much work and communication as possible.
  %However, the choice of concurrency may introduce data-races, and subsequently, fine-grained synchronization.
  %At this junction, we optimize for the remaining communication dimensions, consistency and coherence.

  %For algorithms which implement indirect-pointer jumping or traversal of dynamic graph properties, the optimization space of communication for ACRs is dictated by the AIS such that we cannot statically optimize for control flow.
  %These effects are discussed later in Section~\ref{subsec:optimization-ais}.
  
  %To summarize as shown in Table~\ref{tbl:aaa-ccc}, for algorithms for which we can optimize ACRs, the design space of communication is affected by the presence of data-races.
  %When dealing with data-races, the coupled issues of concurrency and consistency optimization for data-races may be significant depending on the symmetry presented by the ACRs.
  %\vspace{-0.05in}
  \subsubsection{Algorithmic Information}
  \label{subsec:optimization-ai}

  As described in Section~\ref{subsec:taxonomy-ai}, algorithmic information influences the working set size of the workload.
  By specializing for working set size, we aim to minimize the amount of communication done by each thread.

  If the algorithm has asymmetry in the number of loads between a push and pull kernel, we specialize for the raciness dimension~(push or pull) which hoists the largest amount of variables accessed into the outer loop~(see $s$ and $t$ loop body positions in Figure~\ref{alg:push-pull}).
  Doing so amortizes the cost of accessing the outer loop vertex's property by performing them once, instead of once per incident edge. 
  
  When there is symmetry in algorithmic information, no specialization for raciness hoists more accesses.
  Therefore, for symmetric information, graph structure and the other algorithmic properties will factor into specialization decisions.
  %This is because the kernel structure~(see Figure~\ref{alg:push-pull}) using either racy push updates or non-racy pull will not have a significant impact on the amount of loads hoisted to the outer loop of the kernel.
  %Therefore, in the presence of symmetric information, we do not use it to recommend an implementation dimension.
  % This design space is summarized in Table~\ref{tbl:aaa-ccc}.

  %Some care should be made when choosing an implementation with conflicts~(C) as the consistency model may affect locality.
  %For consistency models which block on fine-grained synchronization~(1), we may schedule out the thread performing the atomic access.
  %This may negate any possible benefits of optimizing for AI if when the thread is rescheduled, the data has already been evicted~(Section~\ref{subsubsec:optimization-volume}).
  %This design space is summarized in Table~\ref{tbl:aaa-ccc}

  %However, optimizing with regard to data-races should have more emphasis due to the possible performance overheads of fine-grained synchronization.
  %If there are no data-races after optimization, then it is safe to ignore protocol optimizations concerning fine-grained synchronization.
  %In scenarios where optimization of communication results in data-races in the application, we must consider the overheads of accessing the dataset dictated by the AIRs, particularly for data that is updated.
  %If a lot of data is updated, and the AIRs necessitate that this data is shared across work items, then bypassing the local caches, or obtaining ownership for atomically updated data, depending on the dataset size.
  %This dataset size depends further on the AIS of the workload.

  %To summarize as shown in Table~\ref{tbl:aaa-ccc}, AIRs have some effect on the choice of concurrency due to potential asymmetry in communication requirements.
  %When dealing with data-races, the coherence protocol has a large performance impact when data-races exist in the workload, and lots of shared data needs to be updated via atomics.

  %\subsection{Prioritizing the Communication Space}
  %\label{subsec:optimization-priority}

  %The difficulty of optimization for communication arises from the inter-dependence of each of the algorithmic properties, the components of communication, and their relationship with data-races in the workload.
  %We first discuss the tight coupling of these concepts to simplify optimization when considering our taxonomy's three algorithmic properties.

  %When an algorithmic property or the concurrency component of communication introduces data-races in the program, the optimal design space for the components of communication narrows.
  %This occurs because the presence of data-races requires fine-grained synchronization for DRF programs.
  %Subsequently, the performance implications of the consistency model and coherence protocols with fine-grained synchronization optimizations must be considered.
  %To achieve optimal performance for consistency models, fine-grained synchronization via atomic operations motivates the use of models that are more relaxed with regard to the value an atomic operation can return.
  %For coherence protocols, the optimization space may narrow towards protocols designed to improve locality for fine-grained synchronization~(e.g., via ownership requests for atomic operations).

  %Conversely, if the algorithmic property or the concurrency component of communication dictates that there are no data-races in the program, the optimal design space for the communication narrows away from concerns related to fine-grained synchronization.
  %In such scenarios for DRF programs, no fine-grained synchronization is needed.
  %Thus, the choice of consistency model and coherence protocol is trivialized as there are no atomic operations for which we can relax the ordering, nor are coherence optimizations for atomic operations relevant.

  %Given this insight for the coupling of algorithmic properties and the communication design space, we propose a methodology to prioritize optimization concerns:
  %\begin{enumerate}
  %  \item First, consider the algorithmic properties of the graph workload, and determine the affect on or introduction of data-races.
  %  \item Second, consider the concurrency of communication, whether the it's made relevant by the algorithmic properties of the application, and how the choice of concurrency will further affect data-races.
  %  \item Third, consider the consistency model and coherence protocol with respect to the presence of data races, as determined by prioritization steps 1 and 2.
  %\end{enumerate}

  %\note{Restructure to order AIS, then ACR, then AIR.}

  \subsection{Putting the Model Together}
  \label{subsec:optimization-nav}

  This section briefly expounds on how our workload-driven model prioritizes the competing specialization goals described in Sections~\ref{subsec:optimization-gs} and~\ref{subsec:optimization-ap}.
  Tables~\ref{tbl:aaa-ccc} and~\ref{tbl:gs-ccc} summarize the recommended implementations depending on the algorithmic traversal, control, information, and graph structure of a given workload.
  
  To produce the final implementation across the three dimensions~(raciness, coherence, and consistency), we use a decision flow as follows:
  First we check the algorithmic properties of the application, and compare with the suggestions summarized in Table~\ref{tbl:aaa-ccc}.
  Any suggestions made by this table for coherence and consistency are chosen for specialization for this workload.
  For raciness, if push is recommended, we predict push.
  Now we move on to Table~\ref{tbl:gs-ccc}.
  If no specialization for raciness was previously made, or Pull was recommended, we predict Pull as long as the graph has high locality and low imbalance.
  Otherwise, we predict Push.
  Now, we check if the graph has high imbalance; if so, we predict DRFrlx.
  Next, we finally check if locality is high or volume is medium or low; if so we predict DeNovo.
  Any remaining dimensions not predicted by this point~(which can occur for coherence and consistency) are predicted to be GPU coherence and DRF1, unless we have predicted Pull.
  As described in Section~\ref{sec:comm-design-space}, non-racy updates can interface with GPU coherence and DRF0 with negligible loss in performance, and improved programmability over DRF1.
  
  %To produce the final system implementations across the three dimensions~(synchronization, coherence, and consistency), we use a majority voting scheme.
  %Each system implementation recommended in the table for the workload receives one vote.
  %In the event of a tie for one of the implementation dimensions, the design chosen defaults to using push with DeNovo coherence and DRFrlx for the racy updates, coherence, and consistency, respectively.

  %Figures~\ref{fig:conflicts-flow-chart} and~\ref{fig:gs-flow-chart} summarize this workload-driven design space pruning.
  %If at any point during the following methodology there is an unambiguous design marked as optimal in Table~\ref{tbl:aaa-ccc} or~\ref{tbl:gs-ccc}, then that design dimension is fixed to that optimal for the remainder of the methodology decision flow.
  %\note{Clean up/clarify the flow of this introductory para. Possibly replace/bolster section with a pseudo-code algorithm. Also consider using a set union/intersection approach for GS~(more holistic).}

  %\subsubsection{Algorithmic Properties}
  %\label{subsubsec:optimization-conflicts}

  %\input{figures-v6/conflicts-flow-chart.tex}

  %The AT property of the workload determines whether we must optimize our workload with conflicts in mind.
  %As described in Section~\ref{subsec:optimization-at}, if the workload has dynamic AT, then we should optimize for the possible presence of conflicts.
  %On the other hand, if the AT is static and our workload is vertex-centric, we still have the choice to optimize for conflicts depending on other workload properties.
  %Therefore, analysis of the applications AT is the first step in our optimization methodology.

  %We then move on to the AC and AI properties of the application.
  %If the AT is dynamic, the AC and AI of the workload will depend on the algorithm and the graph structure properties~(as discussed in Section~\ref{subsec:optimization-at}).
  %Otherwise, we focus on optimizing for the AC and AI of our static AT workload.

  %Both the AC and the AI of the workload can favor either no conflicts, conflicts, or neither design.
  %Given that successful optimization for the AC can cause entire loop iterations to be elided, we optimize for the applications AC conflicts preference first.
  %For example, if the AC favors conflicts, we only consider the design points in Table~\ref{tbl:aaa-ccc} that our analysis states is optimal for conflicts.
  %In the case that the AC for the algorithm is symmetrically preferred, we subsequently perform a similar design space pruning for AI.
  %If the static AT workload also symmetrically prefers AI, then we choose the optimal communication design point based on the input graph's GS.
  
  %This methodology is shown in Figure~\ref{fig:conflicts-flow-chart}.

  %\subsubsection{Graph Structure}
  %\label{subsubsec:optimization-gs}

  %\input{figures-v6/gs-flow-chart.tex}

  %Once we have optimized for conflicts as described in Section~\ref{subsubsec:optimization-conflicts}, we need to optimize for the input graph's GS either apriori or at runtime.
  %Based on the interplay of GS and communication performance described in Section~\ref{subsec:optimization-gs}, we optimize our workload from the remaining pool of design points.
  %Then once we compute the volume, locality, and imbalance characteristics of our workload's input, we use Table~\ref{tbl:gs-ccc} to finalize the optimal design.

  %As for conflicts, we need to distinguish which design points should be chosen by the methodology in the presence of competing optimization goals.
  %Therefore, we prioritize volume, locality, and imbalance for the remaining designs available in Table~\ref{tbl:gs-ccc} by following the flow chart in Figure~\ref{fig:gs-flow-chart}.
  %First, we prioritize by imbalance.
  %This is because the SIMT architecture of GPUs can cause imbalanced workloads to have the most dramatic impact on kernel performance~(when long latency warps cause thread blocks to hold resources),
  %Next, we prioritize by locality, which can provide ample opportunities for decreasing the volume communication of a workload.
  %Lastly, we choose the optimal design point based on volume.
  %If at the end there are still unchosen designs for dimensions of the communication design space, we choose the design closest to CGR for the remaining dimensions.

  %AC is only important when a choice exists between C and N.
  %While minimizing the amount of work done via AC is more likely to have a larger impact on performance, we should still consider how AI affects the optimal design for communication.

  %\subsection{Concurrency}
  %\label{subsec:optimization-concurrency}

  %\subsection{Consistency}
  %\label{subsec:optimization-consistency}

  %\subsection{Coherence}
  %\label{subsce:optimization-coherence}


==> results2.tex <==
\section{Evaluation}
\label{sec:results}

\input{figures-v6/stalls.tex}

Performance results for the evaluated applications, configurations, and input graphs described in Section~\ref{sec:methodology} are shown in Figure~\ref{fig:results}.
Each bar represents the GPU execution time normalized to the leftmost configuration --- CG1 for CC, and NG1 for all other applications.
Each bar is subdivided into one of five execution time components using a stall classification methodology similar to that described by Alsop et al.~\cite{AlsopSinclair2016}.
\textit{Busy} represents time spent doing useful work~(cycles where 1 or more instructions were able to issue). 
\textit{Comp} represents time spent waiting for an occupied computation unit or the result of a computation.
\textit{Data} represents time spent waiting for an occupied LD/ST unit, or waiting for the result of a non-atomic memory operation.
\textit{Sync} represents time spent waiting for the result of an atomic memory operation, or waiting at a thread barrier.
\textit{Idle} represents idle time spent by a GPU core as it waits for other cores to complete a kernel.

    % \subsection{Overall Trends}
    % \label{subsec:results-overall}
    
    %Point 1
    %There is no one config that does the best (even for one app or one graph??)
    
    %Point 2
    %We have a methodology that predicts the best config given graph+app
    
    % \subsection{Flexibility Matters}
    % \label{subsec:results-flex}
    
The first key takeaway from our results is that a one size fits all approach can lead to suboptimal performance in certain cases.
% while some system implementations perform well across many applications and evaluated graphs, using a singular design for all possible application and graph combinations can lead to suboptimal performance.
We observe that while CGR performs well for a majority of the workloads, it is not the optimal design in XXX application and graph combinations, as illustrated in Figure~\ref{fig:cgr}.
These combinations span a variety of applications and input graphs, and the best configuration in these combinations is significantly faster than CGR (YYY\% on average, max ZZZ\%).
Furthermore, \emph{the design predicted by our methodology is always the best design in these cases}.
This motivates the use of our methodology in order to select the best performing configuration for a given application and graph input pair.

% The first takeaway for this work is that while some system implementations perform well across many applications and graphs evaluated, using a singular design for all possible application and graph combinations can lead to suboptimal performance.
% We observe that the CGR design performs well for a majority of the workloads. 
% However, Figure~\ref{fig:cgr} illustrates the difference in performance gained over CGR by using a different design, if the system could reconfigure to other implementations for the given workload.

    % \subsection{Methodology Success}
    % \label{subsec:results-meth}
    
The second major takeaway from our results is that our proposed methodology is highly successful at predicting the best configuration for a given graph workload.
As shown in Table~\ref{tbl:designs}, our methodology correctly predicts XXX out of YYY designs.
Furthermore, ZZZ out of YYY designs perform similarly to the optimal and are less than 5\% slower.
As shown in Figure~\ref{fig:results}, for five out of the six evaluated applications, the empirically best configurations only reduce execution time by less than 1.35\% (0.59\% on average) compared to our methodology's predicted designs.
For CC, the empirically best configurations reduce execution time by 17.5\% on average compared to our methodology.
However, this is due to a performance regression in the simulated system, as described in Section~\ref{subsec:results-methodology}.

% The second major takeaway for this work is that we propose a methodology that is successful at capturing the salient features of graph workloads which can cause performance issues in current GPU systems.
% Section~\ref{subsec:results-meth} illustrates that there are combinations of application and graph inputs for which having a rigid, non-configurable memory system can lead to suboptimal performance.
% On the other hand, our methodology shows that if we design systems with a flexible software-hardware interface, we can achieve close to the empirically found optimal performance for the large majority of the workload combinations evaluated.

% For 5 of the 6 applications evaluated, the empirical best combination of designs only reduces execution times by less than 1.35\% over our methodology's predicted designs~(0.59\% on average).
% For the CC application, the best combination of designs reduces executions times by less than 68.64\% over our methodology~(17.15\% on average).
% While the efficacy of the methodology is notably worse for the CC application relative to the other applications, this can be explained by a performance regression experienced by the hardware we evaluate when using the CGR design in CC.
% This application is sensitive to the MSHR design we implement because our MSHRs operate on an unordered network interconnect.
% To ensure the correct ordering for RMWs to the same word from the same thread when using DRFrlx~(R), requests to each line in the MSHR are queued.
% However, these RMW requests are tracked at the line granularity for all threads on a core, and L2 RMWs cannot be coalesced at the L1 MSHR.
% Therefore, designs for CC using both DRFrlx~(R) and GPU coherence~(G) suffer when there are no true dependencies between RMWs of different threads at the same core, and the requests are to the same line.

==> tables/aaa-ccc.tex <==
\begin{table}[!ht]
  \centering
  \captionsetup{font=footnotesize}
  \caption{Graph Structure based implementation specialization.
           The recommended design for each workload property is shown in the cell for that dimension.
           A `\okay' marks where other information about the workload is needed to make a specialization determination for a given dimension.}
%\begin{subtable}[t]{0.46\textwidth}
  \scriptsize
  \begin{tabular}[t]{ l | l | c  c  c }
  \toprule
  \textbf{Structure}    & \textbf{Classification}    & \textbf{Raciness}    & \textbf{Coherence}    & \textbf{Consistency}      \\
  \midrule                                                               
                        & \textcolor{red}{High}      & Push                 & GPU                   & \okay            \\
  \mline{Volume}        & \textcolor{orange}{Medium} & \okay                & GPU                   & \okay            \\
                        & \textcolor{blue}{Low}      & \okay                & DeNovo                & \okay            \\
  \midrule                                             
                        & \textcolor{blue}{High}     & \okay                & DeNovo                & \okay            \\
  \mline{Locality}      & \textcolor{orange}{Medium} & \okay                & \okay                 & \okay            \\
                        & \textcolor{red}{Low}       & Push                 & GPU                   & \okay            \\
  \midrule                                              
                        & \textcolor{red}{High}      & Push                 & \okay                 & DRFrlx           \\
  \mline{Imbalance}     & \textcolor{orange}{Medium} & \okay                & \okay                 & \okay            \\
                        & \textcolor{blue}{Low}      & \okay                & \okay                 & \okay            \\
  \bottomrule
  \end{tabular}%
  \normalsize
  %\centering
  %\vspace{0.4cm}
  %\caption{Graph Structure}
  %\begin{tabular}{ l || l l | l l | l l }
  %    & Volume \textcolor{red}{High}    & Volume \textcolor{blue}{Low}  & Locality \textcolor{blue}{High}   & Locality \textcolor{red}{Low} & Imbalance \textcolor{red}{High}   & Imbalance \textcolor{blue}{Low}   \\
  %  \hline
  %  G & \yes                            & \no                           & \yes / \no                        & \yes                          & \yes / \no                        & \okay            \\
  %  D & \no                             & \yes                          & \no / \yes                        & \no                           & \no / \yes                        & \okay            \\
  %  \hline
  %  1 & \okay                           & \no                           & \yes / \okay                      & \okay                         & \yes / \no                        & \okay            \\
  %  R & \okay                           & \yes                          & \no / \okay                       & \okay                         & \no / \yes                        & \okay            
  %\end{tabular}%
  \label{tbl:gs-ccc}%
\end{table}%
%\hspace{\fill}
\begin{table}[ht]
%\begin{subtable}[t]{0.53\textwidth}
  %\flushright
  \centering
  %\caption{Algorithmic properties and system implementation design space.
  %         The recommended system design for each algorithmic property is shown in the cell for that implementation dimension.}
    \captionsetup{font=footnotesize}
  \caption{Algorithmic Property based implementation specialization.
           The recommended system design for each workload property is shown in the cell for that dimension.
           A `\okay' marks where other information about the workload is needed to make a specialization determination for a given dimension.}
  \scriptsize
  \begin{tabular}[t]{ l | l | c  c  c }
  \toprule
  \textbf{Property}     & \textbf{Classification}    & \textbf{Raciness}    & \textbf{Coherence}    & \textbf{Consistency}     \\
  \midrule
                        & \DynWI                     & Push+Pull            & DeNovo                   & DRF1            \\
  \mline{Traversal}     & \DynWO                     & Push+Pull            & DeNovo                & DRF1            \\
                        & Static                     & \okay                & \okay                 & \okay           \\
  \midrule
                        & \PullAC                    & Pull                 & \okay                 & \okay           \\
  \mline{Control}       & Symmetric                  & \okay                & \okay                 & \okay           \\
                        & \PushAC                    & Push                 & \okay                 & \okay           \\
  \midrule
                        & \PullAI                    & Pull                 & \okay                 & \okay           \\
  \mline{Information}   & Symmetric                  & \okay                & \okay                 & \okay           \\
                        & \PushAI                    & Push                 & \okay                 & \okay           \\
  \bottomrule
  \end{tabular}%
  \normalsize
  %\centering
  %\vspace{0.4cm}
  %\caption{Algorithmic Properties}
  %\scriptsize
  \label{tbl:aaa-ccc}%
\end{table}%
  %\begin{tabular}{ l || c | c || c | c }
  %                                          & G             & D             & 1             & R             \\
  %  \hline
  %  AT is Dynamic w/ increasing conflicts   & \yes          & \no           & \no           & \yes          \\
  %  AT is Dynamic w/o increasing conflicts  & \no           & \yes          & \no           & \yes          \\
  %  AT is Static                            & \okay         & \okay         & \okay         & \okay         \\
  %  \hline
  %  AC Favors No Conflicts                  & \yes          & \no           & \yes          & \no           \\
  %  AC is Symmetric                         & \okay         & \okay         & \okay         & \okay         \\
  %  AC Favors Conflicts                     & \okay         & \okay         & \no           & \yes          \\
  %  \hline
  %  AI Favors No Conflicts                  & \yes          & \no           & \yes          & \no           \\
  %  AI is Symmetric                         & \okay         & \okay         & \okay         & \okay         \\
  %  AI Favors Conflicts                     & \okay         & \okay         & \no           & \yes          
  %\end{tabular}%
  %\normalsize
%%   %\caption{Interaction of communication design space~(Section~\ref{sec:comm-design-space}) and workload properties~(Section~\ref{sec:optimization}).
%%   %         Each design point is specified as conflict+coherence+consistency. Red, blue, and green map to low, medium, and high levels for each GS property.}%
%% %   \begin{tabular}{c c c c c}
%% %     \textbf{Cf+Cs+Ch}     & \textbf{GS}   & \textbf{AT}   & \textbf{AC}   & \textbf{AI}  \\
%% %     \hline
%% %     Pl+0+L2               & \yes          & \no           & \yes          & \yes         \\
%% %     Pu+1+L2               & \yes          & \no           & \yes          & \yes         \\
%% %     Pu+1+Oa               & \yes          & \no           & \yes          & \yes         \\
%% %     Pu+R+L2               & \yes          & \no           & \yes          & \yes         \\
%% %     Pu+R+Oa               & \yes          & \no           & \yes          & \yes         \\
%% %     PP+1+L2               & \yes          & \yes          & \no           & \no          \\
%% %     PP+1+Oa               & \yes          & \yes          & \no           & \no          \\
%% %     PP+R+L2               & \yes          & \yes          & \no           & \no          \\
%% %     PP+R+Oa               & \yes          & \yes          & \no           & \no   
%% %   \end{tabular}
%%   \begin{tabular}{c c c c c}
%%     \textbf{Design Point}     & \textbf{S/Pu/*}   & \textbf{S/Pl/*}   & \textbf{S/Sym/Sym}   & \textbf{S/Sym/Pu}  \\
%%     \hline
%%     NG1               & \yes          & \no           & \yes          & \yes         \\
%%     CG1               & \yes          & \no           & \yes          & \yes         \\
%%     CGR               & \yes          & \no           & \yes          & \yes         \\
%%     CD1               & \yes          & \no           & \yes          & \yes         \\
%%     CDR               & \yes          & \no           & \yes          & \yes         \\
%% %    PP+1+L2               & \yes          & \yes          & \no           & \no          \\
%% %    PP+1+Oa               & \yes          & \yes          & \no           & \no          \\
%% %    PP+R+L2               & \yes          & \yes          & \no           & \no          \\
%% %    PP+R+Oa               & \yes          & \yes          & \no           & \no   
%%   \end{tabular}%
%%   %\begin{tabular}{l l l l}
%%   %          & Concurrency                 & Consistency                 & Coherence                 \\ \hline
%%   %  ACR     & \textcolor{red}{High}       & \textcolor{red}{High}       & \textcolor{green}{Low}    \\
%%   %  AIR     & \textcolor{orange}{Medium}  & \textcolor{green}{Low}      & \textcolor{red}{High}     \\
%%   %  AIS     & \textcolor{red}{High}       & \textcolor{red}{High}       & \textcolor{orange}{Medium}    
%%   %\end{tabular}
%\end{table*}%


==> tables/configurations.tex <==
\begin{table}[!t]
  \centering
  %\captionsetup{justification=centering,labelfont=bf}
  \captionsetup{font=footnotesize}
  \caption{Implementation abbreviations for design space~(described in Section~\ref{sec:comm-design-space}).}%
  %\vspace{-1.5ex}
  %\footnotesize
  \scriptsize
  \begin{tabular}{ c c | }
  	\toprule
    \textbf{Abbr.}  & \textbf{Push/Pull}        \\
    \midrule
      \textbf{T}    & \textbf{T}arget centric   \\
      \textbf{S}    & \textbf{S}ource centric \\
      \textbf{D}    & \textbf{D}ynamic \\
    \bottomrule
  \end{tabular}%
  \begin{tabular}{ c c | }
  	\toprule
    \textbf{Abbr.}  & \textbf{Coherence}        \\
    \midrule
      \textbf{G}    & \textbf{G}PU    \\
      \textbf{D}    & \textbf{D}eNovo \\
                    &                 \\
    \bottomrule
  \end{tabular}%
  \begin{tabular}{ c c }
  	\toprule
    \textbf{Abbr.}  & \textbf{Consistency}      \\
    \midrule
      \textbf{0}    & DRF\textbf{0} \\
      \textbf{1}    & DRF\textbf{1} \\
      \textbf{R}    & DRF\textbf{r}lx \\
    \bottomrule
  \end{tabular}%
  %\begin{tabular}{ c c }
  %	\toprule
  %  \textbf{Name} & \textbf{Description} \\
  %  \bottomrule
  %    \textbf{N}    & \textbf{N}on-racy pull \\
  %    \textbf{C}    &  Ra\textbf{c}y push/pull \\
  %  \midrule
  %    \textbf{G}    & \textbf{G}PU coherence    \\
  %    \textbf{D}    & \textbf{D}eNovo \\
  %  \midrule
  %    \textbf{0}    & DRF\textbf{0} \\
  %    \textbf{1}    & DRF\textbf{1} \\
  %    \textbf{R}    & DRF\textbf{r}lx \\
  %  \bottomrule
  %\end{tabular}%
  %\begin{tabular}{ c c }
  %	\hline
  %  \textbf{Name} & \textbf{Description} \\
  %  \hline
  %    NG1    & \mline{Non-racy pull updates + GPU Coherence + DRF1} \\
  %  \hline
%       G0    & GPU Coherence + DRF0 + L2 Atomics \\
%       G1    & GPU Coherence + DRF1 + L2 Atomics \\
%       GR    & GPU Coherence + DRFrlx + L2 Atomics \\
  %    CG1    & \mline{Racy push/pull updates + GPU Coherence + DRF1} \\
  %    CGR    & \mline{Racy push/pull updates + GPU Coherence + DRFrlx} \\
  %    %\hline
  %    %D0    & DeNovo Coherence + Data-Race-Free-0 + L2 Atomics \\
  %    %D1    & DeNovo Coherence + Data-Race-Free-1 + L2 Atomics \\
  %    %D2    & DeNovo Coherence + Data-Race-Free-2 + L2 Atomics \\
  %    \hline
%       D0    & DeNovo Coherence + DRF0 + Owned Atomics \\
%       D1    & DeNovo Coherence + DRF1 + Owned Atomics \\
%       DR    & DeNovo Coherence + DRFrlx + Owned Atomics \\
   %   CD1    & \mline{Racy push/pull updates + DeNovo Coherence + DRF1} \\
   %   CDR    & \mline{Racy push/pull updates + DeNovo Coherence + DRFrlx} \\
   %  \hline
  %\end{tabular}%
  \normalsize
  \label{tbl:configs}%
\end{table}%


==> tables/gs-ccc.tex <==
\begin{table}[!ht]
  \centering
  \caption{Graph Structure and system implementation design space.
           The recommended system design for each algorithmic property is shown in the cell for that implementation dimension.}
  \small
  \begin{tabular}{ l || l || c | c | c }
  Feature               & Classification             & Raciness     & Coherence     & Consistency      \\
  \hline                                                               
                        & \textcolor{red}{High}      & Push         & GPU           & \okay            \\
  \mline{Volume}        & \textcolor{orange}{Medium} & \okay        & GPU           & \okay            \\
                        & \textcolor{blue}{Low}      & \okay        & DeNovo        & \okay            \\
  \hline                                              
                        & \textcolor{blue}{High}     & \okay        & DeNovo        & \okay            \\
  \mline{Locality}      & \textcolor{orange}{Medium} & \okay        & \okay         & \okay            \\
                        & \textcolor{red}{Low}       & Push         & GPU           & \okay            \\
  \hline                                              
                        & \textcolor{red}{High}      & \okay        & \okay         & DRFrlx           \\
  \mline{Imbalance}     & \textcolor{orange}{Medium} & \okay        & \okay         & \okay            \\
                        & \textcolor{blue}{Low}      & \okay        & \okay         & \okay             
  \end{tabular}%
  \normalsize
  %\begin{tabular}{ l || l l | l l | l l }
  %    & Volume \textcolor{red}{High}    & Volume \textcolor{blue}{Low}  & Locality \textcolor{blue}{High}   & Locality \textcolor{red}{Low} & Imbalance \textcolor{red}{High}   & Imbalance \textcolor{blue}{Low}   \\
  %  \hline
  %  G & \yes                            & \no                           & \yes / \no                        & \yes                          & \yes / \no                        & \okay            \\
  %  D & \no                             & \yes                          & \no / \yes                        & \no                           & \no / \yes                        & \okay            \\
  %  \hline
  %  1 & \okay                           & \no                           & \yes / \okay                      & \okay                         & \yes / \no                        & \okay            \\
  %  R & \okay                           & \yes                          & \no / \okay                       & \okay                         & \no / \yes                        & \okay            
  %\end{tabular}%
  \label{tbl:gs-ccc}%
\end{table}%


==> tables/inputs-classification.tex <==
\begin{table}[!ht]
  \centering
  \small
  \captionsetup{font=footnotesize}
  \caption{Graph Structure profile of each input graph.
  % consisting of data volume, anticipated locality and imbalance. 
  \textcolor{blue}{Blue} classifications 
  % (low volume, high locality, low imbalance) 
  indicate 
  favorable characteristics and \textcolor{red}{red} ones indicate negative characteristics.}
  \begin{tabular}{ l | l l l }
    \toprule
    \textbf{Graph}    & \textbf{Volume}               & \textbf{Locality}             & \textbf{Imbalance}          \\
    \midrule
    AMZ               & \textcolor{red}{High}         & \textcolor{orange}{Medium}    & \textcolor{blue}{Low}       \\
    DCT               & \textcolor{orange}{Medium}    & \textcolor{orange}{Medium}    & \textcolor{orange}{Medium}  \\
    EML               & \textcolor{red}{High}         & \textcolor{red}{Low}          & \textcolor{red}{High}       \\
    OLS               & \textcolor{orange}{Medium}    & \textcolor{blue}{High}        & \textcolor{blue}{Low}       \\
    RAJ               & \textcolor{blue}{Low}         & \textcolor{blue}{High}        & \textcolor{red}{High}       \\
    WNG               & \textcolor{orange}{Medium}    & \textcolor{red}{Low}          & \textcolor{blue}{Low}       \\
    \bottomrule
  \end{tabular}%
  \label{tbl:input-classification}%
\end{table}%


==> tables/inputs.tex <==
%\begin{table*}[!t]
%  \centering
%  %\captionsetup{justification=centering,labelfont=bf}
%  \caption{Input Graph Connectivity Properties}
%  %\vspace{0.5cm}
%  \tiny
%  \begin{tabular}{ c c c c c c c c }
%    \hline
%    \textbf{Name} & \textbf{Vertices} & \textbf{Avg. Degree} & \textbf{Max. Degree} & \textbf{Local Neighbors} & \textbf{Shared Local Neighbors} & \textbf{Shared Remote Neighbors} \\
%    \hline
%    Rajat27~(R27) 		& 20640 & 7.91 & 3469 	& 4.70 & 6.30 	& 7.91 \\
%    %\hline
%    Dictionary28~(D28) 	& 52652 & 3.38 & 38 	& 1.22 & 1.54 	& 3.38 \\
%    %\hline
%    Wing~(WN) 			& 62032 & 3.92 & 4 		& 0.02 & 0.07  	& 3.92 \\
%    %\hline
%    Olesnik0~(OK0) 		& 88263 & 7.74 & 10 	& 3.45 & 7.05 	& 7.74 \\
%    \hline
%  \end{tabular}
%  \normalsize
%  \label{tbl:inputs}
%\end{table*}
\input{tables/stats-basic.tex}
\input{tables/stats-locality.tex}


==> tables/stats-basic.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[!t]
  \centering
  \scriptsize
  \captionsetup{font=footnotesize}
  \caption{General input graph connectivity statistics.}%
  \begin{tabular}{ l | r r r r r r r }
    %\multicolumn{1}{p{1.5em}}{\textbf{Graph}} & \multicolumn{1}{p{4.235em}}{\textbf{Vertices}} & \multicolumn{1}{p{2.5em}}{\textbf{Edges}} & \multicolumn{1}{p{2.5em}}{\textbf{Max Deg}} & \multicolumn{1}{p{1.5em}}{\textbf{Avg Deg}} & \multicolumn{1}{p{4.235em}}{\textbf{Std Dev Deg}} \\ \hline \vspace{0.1cm}
      \toprule
    \textbf{Graph} & \textbf{Vertices} & \textbf{Edges} & \textbf{Max Deg} & \textbf{Avg Deg} & \textbf{Std Dev Deg} \\
      \midrule
      AMZ   & 410236    & 6713648   & 2770    & 16.365    & 16.298      \\
      DCT   & 52652     & 178076    & 38      & 3.382     & 4.475       \\
      EML   & 265214    & 837912    & 7636    & 3.159     & 42.490      \\
      OLS   & 88263     & 683186    & 10      & 7.740     & 2.411       \\
      RAJ   & 20640     & 163178    & 3469    & 7.906     & 32.954      \\
      WNG   & 62032     & 243088    & 4       & 3.919     & 0.278       \\
      \bottomrule
  \end{tabular}%
  \normalsize
  \label{tbl:stats-basic}%
\end{table}%


==> tables/stats-locality.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[!t]
  \centering
  \captionsetup{font=footnotesize}
  \caption{Input graph structure statistics for volume, locality, and imbalance.}%
  \scriptsize
  \begin{tabular}{ l | r r r r r r }
      \toprule
      \textbf{Graph}    & \textbf{Volume}~(KB)  & $\mathbf{AN_L}$   & $\mathbf{AN_R}$   & \textbf{Locality} & \textbf{Imbalance}    \\
      \midrule
      AMZ               & 1855.178              & 2.616             & 13.749            & 0.160             & 0.000                 \\
      DCT               & 60.078                & 1.215             & 2.167             & 0.359             & 0.083                 \\
      EML               & 287.272               & 0.167             & 2.992             & 0.053             & 1.000                 \\
      OLS               & 200.898               & 3.446             & 4.295             & 0.445             & 0.000                 \\
      RAJ               & 47.869                & 4.697             & 3.209             & 0.594             & 0.617                 \\
      WNG               & 79.458                & 0.020             & 3.899             & 0.005             & 0.000                 \\
      \bottomrule
   \end{tabular}%
   %\begin{tabular}{lrrrrrr}
   %   \multicolumn{1}{p{1.5em}}{\textbf{Graph}} & \multicolumn{1}{p{2.5em}}{$\mathbf{AN_L}$} & \multicolumn{1}{p{2.5em}}{$\mathbf{AN_R}$} & \multicolumn{1}{p{3.0em}}{$\mathbf{ANS_L}$} & \multicolumn{1}{p{3.0em}}{$\mathbf{ANS_R}$} & \multicolumn{1}{p{4.235em}}{\textbf{Imbalance}} \\ \hline \vspace{0.1cm}
   %   AMZ & 2.616     & 13.749      & 38.953      & 469.173     & 0.000     \\
   %   DCT & 1.215     & 2.167       & 5.263       & 22.815      & 0.083     \\
   %   EML & 0.167     & 2.992       & 9.288       & 1802.110    & 1.000     \\
   %   OLS & 3.446     & 4.295       & 22.950      & 35.037      & 0.000     \\
   %   RAJ & 4.697     & 3.209       & 227.675     & 905.265     & 0.617     \\
   %   WNG & 0.020     & 3.899       & 0.070       & 11.446      & 0.000     
   %\end{tabular}%
   \normalsize
  \label{tbl:stats-locality}%
\end{table}%
%      (AMZ) amazon0505 		& 2.616     & 13.749      & 187.082     & 38.953      & 494.483     & 0.000     \\
%      (DCT) dictionary28 	& 1.215     & 2.167       & 34.880      & 5.263       & 26.198      & 0.083     \\
%      (EML) email\_EuAll 	& 0.167     & 2.992       & 4.627       & 9.288       & 1806.090    & 1.000     \\
%      (OLS) olesnik0 		& 3.446     & 4.295       & 189.639     & 22.950      & 42.778      & 0.000     \\
%      (RAJ) rajat27 		& 4.697     & 3.209       & 296.548     & 227.675     & 920.801     & 0.617     \\
%      (WNG) wing 			& 0.020     & 3.899       & 0.824       & 0.070       & 15.364      & 0.000     

